The DES Bright Arcs Survey: Candidate Strongly Lensed Galaxy Systems from the Dark Energy Survey 5,000 Sq. Deg. Footprint

We report the combined results of eight searches for strong gravitational lens systems in the full 5,000 sq. deg. of Dark Energy Survey (DES) observations. The observations accumulated by the end of the third observing season fully covered the DES footprint in 5 filters (grizY), with an $i-$band limiting magnitude (at $10\sigma$) of 23.44. In four searches, a list of potential candidates was identified using a color and magnitude selection from the object catalogs created from the first three observing seasons. Three other searches were conducted at the locations of previously identified galaxy clusters. Cutout images of potential candidates were then visually scanned using an object viewer. An additional set of candidates came from a data-quality check of a subset of the color-coadd "tiles" created from the full DES six-season data set. A short list of the most promising strong lens candidates was then numerically ranked according to whether or not we judged them to be bona fide strong gravitational lens systems. These searches discovered a diverse set of 247 strong lens candidate systems, of which 81 are identified for the first time. We provide the coordinates, magnitudes, and photometric properties of the lens and source objects, and an estimate of the Einstein radius for 81 new systems and 166 previously reported. This catalog will be of use for selecting interesting systems for detailed follow-up, studies of galaxy cluster and group mass profiles, as well as a training/validation set for automated strong lens searches.

==> cutouts-placehold.tex <==
\begin{figure}[ht]
\begin{center}
\missingfigure{}
\caption{First page of SL systems with rank 3 or more.   Each cutout image has the visual inspection ranking displayed in a red box in the lower right hand corner. All images are oriented north up, east left.  Each cutout is dynamically sized to fit the SL system well within the cutout, with a minimum size of 30\arcsec \ $\times$ 30\arcsec \ .  A scale bar 10\arcsec \ long is displayed in the lower left hand corner. }
\label{fig:cutouts-1}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\missingfigure{}
\caption{Second page of SL systems with rank 3 or more.   Each cutout image has the visual inspection ranking displayed in a red box in the lower right hand corner. All images are oriented north up, east left.  Each cutout is dynamically sized to fit the SL system well within the cutout, with a minimum size of 30\arcsec \ $\times$ 30\arcsec \ .  A scale bar 10\arcsec \ long is displayed in the lower left hand corner. }
%\label{fig:cutouts-2}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\missingfigure{}
\caption{Third page of SL systems with rank 3 or more.   Each cutout image has the visual inspection ranking displayed in a red box in the lower right hand corner. All images are oriented north up, east left.  Each cutout is dynamically sized to fit the SL system well within the cutout, with a minimum size of 30\arcsec \ $\times$ 30\arcsec \ .  A scale bar 10\arcsec \ long is displayed in the lower left hand corner. }
%\label{fig:cutouts-3}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\missingfigure{}
\caption{Fourth page of SL systems with rank 3 or more.   Each cutout image has the visual inspection ranking displayed in a red box in the lower right hand corner. All images are oriented north up, east left.  Each cutout is dynamically sized to fit the SL system well within the cutout, with a minimum size of 30\arcsec \ $\times$ 30\arcsec \ .  A scale bar 10\arcsec \ long is displayed in the lower left hand corner. }
%\label{fig:cutouts-4}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\missingfigure{}
\caption{Fifth page of SL systems with rank 3 or more.   Each cutout image has the visual inspection ranking displayed in a red box in the lower right hand corner. All images are oriented north up, east left.  Each cutout is dynamically sized to fit the SL system well within the cutout, with a minimum size of 30\arcsec \ $\times$ 30\arcsec \ .  A scale bar 10\arcsec \ long is displayed in the lower left hand corner. }
%\label{fig:cutouts-5}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\missingfigure{}
\caption{Sixth page of SL systems with rank 3 or more.   Each cutout image has the visual inspection ranking displayed in a red box in the lower right hand corner. All images are oriented north up, east left.  Each cutout is dynamically sized to fit the SL system well within the cutout, with a minimum size of 30\arcsec \ $\times$ 30\arcsec \ .  A scale bar 10\arcsec \ long is displayed in the lower left hand corner. }
%\label{fig:cutouts-6}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\missingfigure{}
\caption{Seventh page of SL systems with rank 3 or more.   Each cutout image has the visual inspection ranking displayed in a red box in the lower right hand corner. All images are oriented north up, east left.  Each cutout is dynamically sized to fit the SL system well within the cutout, with a minimum size of 30\arcsec \ $\times$ 30\arcsec \ .  A scale bar 10\arcsec \ long is displayed in the lower left hand corner. }
%\label{fig:cutouts-7}
\end{center}
\end{figure}

\begin{figure}[ht]
\begin{center}
\missingfigure{}
\caption{Eighth and last page of SL systems with rank 3 or more.   Each cutout image has the visual inspection ranking displayed in a red box in the lower right hand corner. All images are oriented north up, east left.  Each cutout is dynamically sized to fit the SL system well within the cutout, with a minimum size of 30\arcsec \ $\times$ 30\arcsec \ .  A scale bar 10\arcsec \ long is displayed in the lower left hand corner. }
\label{fig:cutouts-8}
\end{center}
\end{figure}

==> deletedrefs7-20.tex <==
@article{ACTSLMena1,
  title = {Southern {{Cosmology Survey}}. {{II}}. {{Massive Optically Selected Clusters}} from 70 {{Square Degrees}} of the {{Sunyaev}}-{{Zel}}'dovich {{Effect Common Survey Area}}},
  author = {Menanteau, Felipe and Hughes, John P. and Barrientos, L. Felipe and Deshpande, Amruta J. and Hilton, Matt and Infante, Leopoldo and Jimenez, Raul and Kosowsky, Arthur and Moodley, Kavilan and Spergel, David and Verde, Licia},
  year = {2010},
  month = dec,
  volume = {191},
  pages = {340--351},
  issn = {0067-0049},
  doi = {10.1088/0067-0049/191/2/340},
  abstract = {We present a catalog of 105 rich and massive (M{$>$}3 \texttimes{}  1014 M sun) optically selected clusters of galaxies extracted from 70 deg2 of public archival griz imaging from the Blanco 4 m telescope acquired over 45 nights between 2005 and 2007. We use the clusters' optically derived properties to estimate photometric redshifts, optical luminosities, richness, and masses. We complement the optical measurements with archival XMM-Newton and ROSAT X-ray data which provide additional luminosity and mass constraints on a modest fraction of the cluster sample. Two of our clusters show clear evidence for central lensing arcs; one of these has a spectacular large diameter, nearly complete Einstein Ring surrounding the brightest cluster galaxy. A strong motivation for this study is to identify the massive clusters that are expected to display prominent signals from the Sunyaev-Zel'dovich effect (SZE) and therefore be detected in the wide-area millimeter-band surveys being conducted by both the Atacama Cosmology Telescope and the South Pole Telescope. The optical sample presented here will be useful for verifying new SZE cluster candidates from these surveys, for testing the cluster selection function, and for stacking analyses of the SZE data.},
  file = {/home/humphrey/Zotero/storage/36VYPM99/Menanteau et al_2010_Southern Cosmology Survey.pdf},
  journal = {\apjs},
  keywords = {cosmic background radiation,cosmology: observations,galaxies: clusters: general,galaxies: distances and redshifts,large-scale structure of universe}
}

@article{ACTSLMena2,
  title = {The {{Atacama Cosmology Telescope}}: {{ACT}}-{{CL J0102}}-4915 "{{El Gordo}}," a {{Massive Merging Cluster}} at {{Redshift}} 0.87},
  shorttitle = {The {{Atacama Cosmology Telescope}}},
  author = {Menanteau, Felipe and Hughes, John P. and Sif{\'o}n, Crist{\'o}bal and Hilton, Matt and Gonz{\'a}lez, Jorge and Infante, Leopoldo and Barrientos, L. Felipe and Baker, Andrew J. and Bond, John R. and Das, Sudeep and Devlin, Mark J. and Dunkley, Joanna and Hajian, Amir and Hincks, Adam D. and Kosowsky, Arthur and Marsden, Danica and Marriage, Tobias A. and Moodley, Kavilan and Niemack, Michael D. and Nolta, Michael R. and Page, Lyman A. and Reese, Erik D. and Sehgal, Neelima and Sievers, Jon and Spergel, David N. and Staggs, Suzanne T. and Wollack, Edward},
  year = {2012},
  month = mar,
  volume = {748},
  pages = {7},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/748/1/7},
  abstract = {We present a detailed analysis from new multi-wavelength observations of  the exceptional galaxy cluster ACT-CL J0102-4915, likely the most massive, hottest, most X-ray luminous and brightest Sunyaev-Zel'dovich (SZ) effect cluster known at redshifts greater than 0.6. The Atacama Cosmology Telescope (ACT) collaboration discovered ACT-CL J0102-4915 as the most significant SZ decrement in a sky survey area of 755 deg2. Our Very Large Telescope (VLT)/FORS2 spectra of 89 member galaxies yield a cluster redshift, z = 0.870, and velocity dispersion, {$\sigma$}gal = 1321 {$\pm$} 106 km s-1. Our Chandra observations reveal a hot and X-ray luminous system with an integrated temperature of T X = 14.5 {$\pm$} 0.1 keV and 0.5-2.0 keV band luminosity of L X = (2.19 {$\pm$} 0.11) \texttimes{} 1045 h -2 70 erg s-1. We obtain several statistically consistent cluster mass estimates; using empirical mass scaling relations with velocity dispersion, X-ray Y X, and integrated SZ distortion, we estimate a cluster mass of M 200a = (2.16 {$\pm$} 0.32) \texttimes{} 1015 h -1 70 M {$\odot$}. We constrain the stellar content of the cluster to be less than 1\% of the total mass, using Spitzer IRAC and optical imaging. The Chandra and VLT/FORS2 optical data also reveal that ACT-CL J0102-4915 is undergoing a major merger between components with a mass ratio of approximately 2 to 1. The X-ray data show significant temperature variations from a low of 6.6 {$\pm$} 0.7 keV at the merging low-entropy, high-metallicity, cool core to a high of 22 {$\pm$} 6 keV. We also see a wake in the X-ray surface brightness and deprojected gas density caused by the passage of one cluster through the other. Archival radio data at 843 MHz reveal diffuse radio emission that, if associated with the cluster, indicates the presence of an intense double radio relic, hosted by the highest redshift cluster yet. ACT-CL J0102-4915 is possibly a high-redshift analog of the famous Bullet cluster. Such a massive cluster at this redshift is rare, although consistent with the standard {$\Lambda$}CDM cosmology in the lower part of its allowed mass range. Massive, high-redshift mergers like ACT-CL J0102-4915 are unlikely to be reproduced in the current generation of numerical N-body cosmological simulations.},
  file = {/home/humphrey/Zotero/storage/ULU6RRCX/Menanteau et al_2012_The Atacama Cosmology Telescope.pdf},
  journal = {\apj},
  keywords = {cosmic background radiation,cosmology: observations,galaxies: clusters: general,galaxies: clusters: individual: ACT-CL J0102–4915}
}

@article{Menanteau.Sifon.ea2013,
  title = {The {{Atacama Cosmology Telescope}}: {{Physical Properties}} of {{Sunyaev}}-{{Zel}}'dovich {{Effect Clusters}} on the {{Celestial Equator}}},
  shorttitle = {The {{Atacama Cosmology Telescope}}},
  author = {Menanteau, Felipe and Sif{\'o}n, Crist{\'o}bal and Barrientos, L. Felipe and Battaglia, Nicholas and Bond, J. Richard and Crichton, Devin and Das, Sudeep and Devlin, Mark J. and Dicker, Simon and D{\"u}nner, Rolando and Gralla, Megan and Hajian, Amir and Hasselfield, Matthew and Hilton, Matt and Hincks, Adam D. and Hughes, John P. and Infante, Leopoldo and Kosowsky, Arthur and Marriage, Tobias A. and Marsden, Danica and Moodley, Kavilan and Niemack, Michael D. and Nolta, Michael R. and Page, Lyman A. and Partridge, Bruce and Reese, Erik D. and Schmitt, Benjamin L. and Sievers, Jon and Spergel, David N. and Staggs, Suzanne T. and Switzer, Eric and Wollack, Edward J.},
  year = {2013},
  month = mar,
  volume = {765},
  pages = {67},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/765/1/67},
  abstract = {We present the optical and X-ray properties of 68 galaxy clusters  selected via the Sunyaev-Zel'dovich (SZ) effect at 148 GHz by the Atacama Cosmology Telescope (ACT). Our sample, from an area of 504 deg2 centered on the celestial equator, is divided into two regions. The main region uses 270 deg2 of the ACT survey that overlaps with the co-added ugriz imaging from the Sloan Digital Sky Survey (SDSS) over Stripe 82 plus additional near-infrared pointed observations with the Apache Point Observatory 3.5 m telescope. We confirm a total of 49 clusters to z {$\approx$} 1.3, of which 22 (all at z {$>$} 0.55) are new discoveries. For the second region, the regular-depth SDSS imaging allows us to confirm 19 more clusters up to z {$\approx$} 0.7, of which 10 systems are new. We present the optical richness, photometric redshifts, and separation between the SZ position and the brightest cluster galaxy (BCG). We find no significant offset between the cluster SZ centroid and BCG location and a weak correlation between optical richness and SZ-derived mass. We also present X-ray fluxes and luminosities from the ROSAT All Sky Survey which confirm that this is a massive sample. One of the newly discovered clusters, ACT-CL J0044.4+0113 at z = 1.1 (photometric), has an integrated XMM-Newton X-ray temperature of kTX = 7.9 {$\pm$} 1.0 keV and combined mass of M 200a = 8.2+3.3 -2.5 \texttimes{} 1014 h -1 70 M {$\odot$}, placing it among the most massive and X-ray-hot clusters known at redshifts beyond z = 1. We also highlight the optically rich cluster ACT-CL J2327.4-0204 (RCS2 2327) at z = 0.705 (spectroscopic) as the most significant detection of the whole equatorial sample with a Chandra-derived mass of M 200a = 1.9+0.6 -0.4 \texttimes{} 1015 h -1 70 M {$\odot$}, placing it in the ranks of the most massive known clusters like El Gordo and the Bullet Cluster.},
  file = {/home/humphrey/Zotero/storage/T3C6HU8L/Menanteau et al_2013_The Atacama Cosmology Telescope.pdf},
  journal = {\apj},
  keywords = {cosmic background radiation,cosmology: observations,galaxies: clusters: general,galaxies: distances and redshifts,large-scale structure of Universe}
}

@article{meneghetti2013,
  title = {Arc {{Statistics}}},
  author = {Meneghetti, M. and Bartelmann, M. and Dahle, H. and Limousin, M.},
  year = {2013},
  month = aug,
  volume = {177},
  pages = {31--74},
  issn = {0038-6308},
  doi = {10.1007/s11214-013-9981-x},
  abstract = {The existence of an arc statistics problem was at the center of a strong debate in the last fifteen years. With the aim to clarify if the optical depth for giant gravitational arcs by galaxy clusters in the so called concordance model is compatible with observations, several studies were carried out which helped to significantly improve our knowledge of strong lensing clusters, unveiling their extremely complex internal structure. In particular, the abundance and the frequency of strong lensing events like gravitational arcs turned out to be a potentially very powerful tool to trace the structure formation. However, given the limited size of observational and theoretical data-sets, the power of arc statistics as a cosmological tool has been only minimally exploited so far. On the other hand, the last years were characterized by significant advancements in the field, and several cluster surveys that are ongoing or planned for the near future seem to have the potential to make arc statistics a competitive cosmological probe. Additionally, recent observations of anomalously large Einstein radii and concentrations in galaxy clusters have reinvigorated the debate on the arc statistics problem. In this paper, we review the work done so far on arc statistics, focussing on what is the lesson we learned and what is likely to improve in the next years.},
  file = {/home/humphrey/Zotero/storage/7W5F5GRJ/Meneghetti et al. - 2013 - Arc Statistics.pdf;/home/humphrey/Zotero/storage/9BSIGHWP/Meneghetti et al_2013_Arc Statistics.pdf},
  journal = {\ssr},
  keywords = {Cosmology,Galaxy clusters,Gravitational lensing}
}

@article{SPTStan,
  title = {Galaxy {{Clusters Discovered}} with a {{Sunyaev}}-{{Zel}}'dovich {{Effect Survey}}},
  author = {Staniszewski, Z. and Ade, P. A. R. and Aird, K. A. and Benson, B. A. and Bleem, L. E. and Carlstrom, J. E. and Chang, C. L. and Cho, H.-M. and Crawford, T. M. and Crites, A. T. and {de Haan}, T. and Dobbs, M. A. and Halverson, N. W. and Holder, G. P. and Holzapfel, W. L. and Hrubes, J. D. and Joy, M. and Keisler, R. and Lanting, T. M. and Lee, A. T. and Leitch, E. M. and Loehr, A. and Lueker, M. and McMahon, J. J. and Mehl, J. and Meyer, S. S. and Mohr, J. J. and Montroy, T. E. and Ngeow, C.-C. and Padin, S. and Plagge, T. and Pryke, C. and Reichardt, C. L. and Ruhl, J. E. and Schaffer, K. K. and Shaw, L. and Shirokoff, E. and Spieler, H. G. and Stalder, B. and Stark, A. A. and Vanderlinde, K. and Vieira, J. D. and Zahn, O. and Zenteno, A.},
  year = {2009},
  month = aug,
  volume = {701},
  pages = {32--41},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/701/1/32},
  abstract = {The South Pole Telescope (SPT) is conducting a Sunyaev-Zel'dovich (SZ) effect survey over large areas of the southern sky, searching for massive galaxy clusters to high redshift. In this preliminary study, we focus on a 40 deg2 area targeted by the Blanco Cosmology Survey (BCS), which is centered roughly at right ascension 5h30m, declination -53\textdegree{} (J2000). Over two seasons of observations, this entire region has been mapped by the SPT at 95 GHz, 150 GHz, and 225 GHz. We report the four most significant SPT detections of SZ clusters in this field, three of which were previously unknown and, therefore, represent the first galaxy clusters discovered with an SZ survey. The SZ clusters are detected as decrements with greater than 5{$\sigma$} significance in the high-sensitivity 150 GHz SPT map. The SZ spectrum of these sources is confirmed by detections of decrements at the corresponding locations in the 95 GHz SPT map and nondetections at those locations in the 225 GHz SPT map. Multiband optical images from the BCS survey demonstrate significant concentrations of similarly colored galaxies at the positions of the SZ detections. Photometric redshift estimates from the BCS data indicate that two of the clusters lie at moderate redshift (z \textasciitilde{} 0.4) and two at high redshift (z gsim 0.8). One of the SZ detections was previously identified as a galaxy cluster in the optical as part of the Abell supplementary southern cluster catalog and in the X-ray using data from the ROSAT All-Sky Survey (RASS). Potential RASS counterparts (not previously identified as clusters) are also found for two of the new discoveries. These first four galaxy clusters are the most significant SZ detections from a subset of the ongoing SPT survey. As such, they serve as a demonstration that SZ surveys, and the SPT in particular, can be an effective means for finding galaxy clusters.},
  file = {/home/humphrey/Zotero/storage/89KZDHTK/Staniszewski et al_2009_Galaxy Clusters Discovered with a Sunyaev-Zel'dovich Effect Survey.pdf},
  journal = {\apj},
  keywords = {cosmic microwave background,cosmology: observations,galaxies: clusters: general}
}


@article{SPTSong,
  title = {Redshifts, {{Sample Purity}}, and {{BCG Positions}} for the {{Galaxy Cluster Catalog}} from the {{First}} 720 {{Square Degrees}} of the {{South Pole Telescope Survey}}},
  author = {Song, J. and Zenteno, A. and Stalder, B. and Desai, S. and Bleem, L. E. and Aird, K. A. and Armstrong, R. and Ashby, M. L. N. and Bayliss, M. and Bazin, G. and Benson, B. A. and Bertin, E. and Brodwin, M. and Carlstrom, J. E. and Chang, C. L. and Cho, H. M. and Clocchiatti, A. and Crawford, T. M. and Crites, A. T. and {de Haan}, T. and Dobbs, M. A. and Dudley, J. P. and Foley, R. J. and George, E. M. and Gettings, D. and Gladders, M. D. and Gonzalez, A. H. and Halverson, N. W. and Harrington, N. L. and High, F. W. and Holder, G. P. and Holzapfel, W. L. and Hoover, S. and Hrubes, J. D. and Joy, M. and Keisler, R. and Knox, L. and Lee, A. T. and Leitch, E. M. and Liu, J. and Lueker, M. and {Luong-Van}, D. and Marrone, D. P. and McDonald, M. and McMahon, J. J. and Mehl, J. and Meyer, S. S. and Mocanu, L. and Mohr, J. J. and Montroy, T. E. and Natoli, T. and Nurgaliev, D. and Padin, S. and Plagge, T. and Pryke, C. and Reichardt, C. L. and Rest, A. and Ruel, J. and Ruhl, J. E. and Saliwanchik, B. R. and Saro, A. and Sayre, J. T. and Schaffer, K. K. and Shaw, L. and Shirokoff, E. and {\v S}uhada, R. and Spieler, H. G. and Stanford, S. A. and Staniszewski, Z. and Stark, A. A. and Story, K. and Stubbs, C. W. and {van Engelen}, A. and Vanderlinde, K. and Vieira, J. D. and Williamson, R. and Zahn, O.},
  year = {2012},
  month = dec,
  volume = {761},
  pages = {22},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/761/1/22},
  abstract = {We present the results of the ground- and space-based optical and  near-infrared (NIR) follow-up of 224 galaxy cluster candidates detected with the Sunyaev-Zel'dovich (SZ) effect in the 720 deg2 of the South Pole Telescope (SPT) survey completed in the 2008 and 2009 observing seasons. We use the optical/NIR data to establish whether each candidate is associated with an overdensity of galaxies and to estimate the cluster redshift. Most photometric redshifts are derived through a combination of three different cluster redshift estimators using red-sequence galaxies, resulting in an accuracy of {$\Delta$}z/(1 + z) = 0.017, determined through comparison with a subsample of 57 clusters for which we have spectroscopic redshifts. We successfully measure redshifts for 158 systems and present redshift lower limits for the remaining candidates. The redshift distribution of the confirmed clusters extends to z = 1.35 with a median of z med = 0.57. Approximately 18\% of the sample with measured redshifts lies at z {$>$} 0.8. We estimate a lower limit to the purity of this SPT SZ-selected sample by assuming that all unconfirmed clusters are noise fluctuations in the SPT data. We show that the cumulative purity at detection significance {$\xi$} {$>$} 5({$\xi$} {$>$} 4.5) is {$>$}=95\% ({$>$}=70\%). We present the red brightest cluster galaxy (rBCG) positions for the sample and examine the offsets between the SPT candidate position and the rBCG. The radial distribution of offsets is similar to that seen in X-ray-selected cluster samples, providing no evidence that SZ-selected cluster samples include a different fraction of recent mergers from X-ray-selected cluster samples.},
  file = {/home/humphrey/Zotero/storage/IN6Y2QZI/Song et al_2012_Redshifts, Sample Purity, and BCG Positions for the Galaxy Cluster Catalog from.pdf},
  journal = {\apj},
  keywords = {cosmology: observations,galaxies: clusters: general,galaxies: distances and redshifts}
}

@article{sanchez14,
  title = {Photometric Redshift Analysis in the {{Dark Energy Survey Science Verification}} Data},
  author = {S{\'a}nchez, C. and Carrasco Kind, M. and Lin, H. and Miquel, R. and Abdalla, F. B. and Amara, A. and Banerji, M. and Bonnett, C. and Brunner, R. and Capozzi, D. and Carnero, A. and Castander, F. J. and {da Costa}, L. A. N. and Cunha, C. and Fausti, A. and Gerdes, D. and Greisel, N. and Gschwend, J. and Hartley, W. and Jouvel, S. and Lahav, O. and Lima, M. and Maia, M. A. G. and Mart{\'i}, P. and Ogando, R. L. C. and Ostrovski, F. and Pellegrini, P. and Rau, M. M. and Sadeh, I. and Seitz, S. and {Sevilla-Noarbe}, I. and Sypniewski, A. and {de Vicente}, J. and Abbot, T. and Allam, S. S. and Atlee, D. and Bernstein, G. and Bernstein, J. P. and {Buckley-Geer}, E. and Burke, D. and Childress, M. J. and Davis, T. and DePoy, D. L. and Dey, A. and Desai, S. and Diehl, H. T. and Doel, P. and Estrada, J. and Evrard, A. and Fern{\'a}ndez, E. and Finley, D. and Flaugher, B. and Frieman, J. and Gaztanaga, E. and Glazebrook, K. and Honscheid, K. and Kim, A. and Kuehn, K. and Kuropatkin, N. and Lidman, C. and Makler, M. and Marshall, J. L. and Nichol, R. C. and Roodman, A. and S{\'a}nchez, E. and Santiago, B. X. and Sako, M. and Scalzo, R. and Smith, R. C. and Swanson, M. E. C. and Tarle, G. and Thomas, D. and Tucker, D. L. and Uddin, S. A. and Vald{\'e}s, F. and Walker, A. and Yuan, F. and Zuntz, J.},
  year = {2014},
  month = dec,
  volume = {445},
  pages = {1482--1506},
  issn = {0035-8711},
  doi = {10.1093/mnras/stu1836},
  abstract = {We present results from a study of the photometric redshift performance  of the Dark Energy Survey (DES), using the early data from a Science Verification period of observations in late 2012 and early 2013 that provided science-quality images for almost 200 sq. deg. at the nominal depth of the survey. We assess the photometric redshift (photo-z) performance using about 15 000 galaxies with spectroscopic redshifts available from other surveys. These galaxies are used, in different configurations, as a calibration sample, and photo-z's are obtained and studied using most of the existing photo-z codes. A weighting method in a multidimensional colour-magnitude space is applied to the spectroscopic sample in order to evaluate the photo-z performance with sets that mimic the full DES photometric sample, which is on average significantly deeper than the calibration sample due to the limited depth of spectroscopic surveys. Empirical photo-z methods using, for instance, artificial neural networks or random forests, yield the best performance in the tests, achieving core photo-z resolutions {$\sigma$}68 {$\sim$} 0.08. Moreover, the results from most of the codes, including template-fitting methods, comfortably meet the DES requirements on photo-z performance, therefore, providing an excellent precedent for future DES data sets.},
  file = {/home/humphrey/Zotero/storage/KBX25VZZ/Sánchez et al_2014_Photometric redshift analysis in the Dark Energy Survey Science Verification.pdf},
  journal = {\mnras},
  keywords = {Astronomical data bases: surveys,galaxies: distances and redshifts,galaxies: statistics,large-scale structure of Universe}
}

@article{DLS,
  title = {First {{Results}} on {{Shear}}-Selected {{Clusters}} from the {{Deep Lens Survey}}: {{Optical Imaging}}, {{Spectroscopy}}, and {{X}}-{{Ray Follow}}-Up},
  shorttitle = {First {{Results}} on {{Shear}}-Selected {{Clusters}} from the {{Deep Lens Survey}}},
  author = {Wittman, D. and Dell'Antonio, I. P. and Hughes, J. P. and Margoniner, V. E. and Tyson, J. A. and Cohen, J. G. and Norman, D.},
  year = {2006},
  month = may,
  volume = {643},
  pages = {128--143},
  issn = {0004-637X},
  doi = {10.1086/502621},
  abstract = {We present the first sample of galaxy clusters selected on the basis of  their weak gravitational lensing shear. The shear induced by a cluster is a function of its mass profile and its redshift relative to the background galaxies being sheared; in contrast to more traditional methods of selecting clusters, shear selection does not depend on the cluster's star formation history, baryon content, or dynamical state. Because mass is the property of clusters that provides constraints on cosmological parameters, the dependence on these other parameters could induce potentially important biases in traditionally selected samples. Comparison of a shear-selected sample with optically and X-ray-selected samples is therefore of great importance. Here we present the first step toward a new shear-selected sample: the selection of cluster candidates from the first 8.6 deg2 of the 20 deg2 Deep Lens Survey (DLS), and tabulation of their basic properties such as redshifts and optical and X-ray counterparts.},
  file = {/home/humphrey/Zotero/storage/UZ3J6AS2/Wittman et al_2006_First Results on Shear-selected Clusters from the Deep Lens Survey.pdf},
  journal = {\apj},
  keywords = {Cosmology: Gravitational Lensing,Galaxies: Clusters: General,Surveys}
}

@article{Zitrin2013,
  title = {A {{Highly Elongated Prominent Lens}} at z = 0.87: {{First Strong}}-Lensing {{Analysis}} of {{El Gordo}}},
  shorttitle = {A {{Highly Elongated Prominent Lens}} at z = 0.87},
  author = {Zitrin, Adi and Menanteau, Felipe and Hughes, John P. and Coe, Dan and Barrientos, L. Felipe and Infante, Leopoldo and Mandelbaum, Rachel},
  year = {2013},
  month = jun,
  volume = {770},
  pages = {L15},
  issn = {0004-637X},
  doi = {10.1088/2041-8205/770/1/L15},
  abstract = {We present the first strong-lensing (SL) analysis of the galaxy cluster  ACT-CL J0102-4915 (El Gordo), in recent HST/ACS images, revealing a prominent strong lens at a redshift of z = 0.87. This finding adds to the already-established unique properties of El Gordo: it is the most massive, hot, X-ray luminous, and bright Sunyaev-Zeldovich effect cluster at z {$>\sptilde$} 0.6, and the only "bullet"-like merging cluster known at these redshifts. The lens consists of two merging massive clumps, where, for a source redshift of zs \textasciitilde{} 2, each clump exhibits only a small, separate critical area, with a total area of 0.69 {$\pm$} 0.11squ' over the two clumps. For a higher source redshift, zs \textasciitilde{} 4, the critical curves of the two clumps merge together into one bigger and very elongated lens (axis ratio \textasciitilde = 5.5), enclosing an effective area of 1.44 {$\pm$} 0.22squ'. The critical curves continue expanding with increasing redshift so that for high-redshift sources (zs {$>\sptilde$} 9) they enclose an area of \textasciitilde 1.91 {$\pm$} 0.30squ' (effective \texttheta{} e \textasciitilde = 46.''8 {$\pm$} 3.''7) and a mass of 6.09 {$\pm$} 1.04 \texttimes{} 1014 M {$\odot$}. According to our model, the area of high magnification ({$\mu$} {$>$} 10) for such high-redshift sources is sime1.2squ', and the area with {$\mu$} {$>$} 5 is sime2.3squ', making El Gordo a compelling target for studying the high-redshift universe. We obtain a strong lower limit on the total mass of El Gordo, {$>\sptilde$} 1.7 \texttimes{} 1015 M {$\odot$} from the SL regime alone, suggesting a total mass of roughly M 200 \textasciitilde{} 2.3 \texttimes{} 1015 M {$\odot$}. Our results should be revisited when additional spectroscopic and HST imaging data are available.},
  file = {/home/humphrey/Zotero/storage/VN4TNQNU/Zitrin et al_2013_A Highly Elongated Prominent Lens at z = 0.pdf},
  journal = {\apjl},
  keywords = {dark matter,galaxies: clusters: general,galaxies: clusters: individual: ACT-CL J0102-4915}
}

@article{Zitrin.Broadhurst.ea2011,
  title = {The {{Cluster Lensing}} and {{Supernova Survey}} with {{Hubble}} ({{CLASH}}): {{Strong}}-Lensing {{Analysis}} of {{A383}} from 16-Band {{HST}}/{{WFC3}}/{{ACS Imaging}}},
  shorttitle = {The {{Cluster Lensing}} and {{Supernova Survey}} with {{Hubble}} ({{CLASH}})},
  author = {Zitrin, A. and Broadhurst, T. and Coe, D. and Umetsu, K. and Postman, M. and Ben{\'i}tez, N. and Meneghetti, M. and Medezinski, E. and Jouvel, S. and Bradley, L. and Koekemoer, A. and Zheng, W. and Ford, H. and Merten, J. and Kelson, D. and Lahav, O. and Lemze, D. and Molino, A. and Nonino, M. and Donahue, M. and Rosati, P. and {Van der Wel}, A. and Bartelmann, M. and Bouwens, R. and Graur, O. and Graves, G. and Host, O. and Infante, L. and Jha, S. and {Jimenez-Teja}, Y. and Lazkoz, R. and Maoz, D. and McCully, C. and Melchior, P. and Moustakas, L. A. and Ogaz, S. and Patel, B. and Regoes, E. and Riess, A. and Rodney, S. and Seitz, S.},
  year = {2011},
  month = dec,
  volume = {742},
  pages = {117},
  issn = {0004-637X},
  doi = {10.1088/0004-637X/742/2/117},
  abstract = {We examine the inner mass distribution of the relaxed galaxy cluster  A383 (z = 0.189), in deep 16 band Hubble Space Telescope/ACS+WFC3 imaging taken as part of the Cluster Lensing And Supernova survey with Hubble (CLASH) multi-cycle treasury program. Our program is designed to study the dark matter distribution in 25 massive clusters, and balances depth with a wide wavelength coverage, 2000-16000 \AA, to better identify lensed systems and generate precise photometric redshifts. This photometric information together with the predictive strength of our strong-lensing analysis method identifies 13 new multiply lensed images and candidates, so that a total of 27 multiple images of nine systems are used to tightly constrain the inner mass profile gradient, dlog {$\Sigma$}/dlog r \textasciitilde = -0.6 {$\pm$} 0.1 (r {$<$} 160 kpc). We find consistency with the standard distance-redshift relation for the full range spanned by the lensed images, 1.01 {$<$} z {$<$} 6.03, with the higher-redshift sources deflected through larger angles as expected. The inner mass profile derived here is consistent with the results of our independent weak-lensing analysis of wide-field Subaru images, with good agreement in the region of overlap (\textasciitilde 0.7-1 arcmin). Combining weak and strong lensing, the overall mass profile is well fitted by a Navarro-Frenk-White profile with M vir = (5.37+0.70 - 0.63 {$\pm$} 0.26) \texttimes{} 1014 M {$\odot$} h -1 and a relatively high concentration, c vir = 8.77+0.44 - 0.42 {$\pm$} 0.23, which lies above the standard c-M relation similar to other well-studied clusters. The critical radius of A383 is modest by the standards of other lensing clusters, rE \textasciitilde = 16 {$\pm$} 2'' (for zs = 2.55), so the relatively large number of lensed images uncovered here with precise photometric redshifts validates our imaging strategy for the CLASH survey. In total we aim to provide similarly high-quality lensing data for 25 clusters, 20 of which are X-ray-selected relaxed clusters, enabling a precise determination of the representative mass profile free from lensing bias.},
  file = {/home/humphrey/Zotero/storage/SI29GFSW/Zitrin et al_2011_The Cluster Lensing and Supernova Survey with Hubble (CLASH).pdf},
  journal = {\apj},
  keywords = {dark matter,galaxies: clusters: general,galaxies: clusters: individual: A383,galaxies: high-redshift,gravitational lensing: strong}
}


@article{oyaizu08a,
  title = {A {{Galaxy Photometric Redshift Catalog}} for the {{Sloan Digital Sky Survey Data Release}} 6},
  author = {Oyaizu, Hiroaki and Lima, Marcos and Cunha, Carlos E. and Lin, Huan and Frieman, Joshua and Sheldon, Erin S.},
  year = {2008},
  month = feb,
  volume = {674},
  pages = {768--783},
  issn = {0004-637X},
  doi = {10.1086/523666},
  abstract = {We present and describe a catalog of galaxy photometric redshifts  (photo-z's) for the Sloan Digital Sky Survey (SDSS) Data Release 6 (DR6). We use the neural network (NN) technique to calculate photo-z's and the nearest neighbor error (NNE) method to estimate photo-z errors for \textasciitilde 77 million objects classified as galaxies in DR6 with r {$<$} 22. The photo-z and photo-z error estimators are trained and validated on a sample of \textasciitilde 640,000 galaxies that have SDSS photometry and spectroscopic redshifts measured by SDSS, the Two Degree Field, the SDSS Luminous Red Galaxy and Quasi-stellar Object Survey (2SLAQ), the Canada-France Redshift Survey (CFRS), the Canadian Network for Observational Cosmology Field Galaxy Survey (CNOC2), the Team Keck Redshift Survey (TKRS), the Deep Extragalactic Evolutionary Probe (DEEP), and DEEP2. For the two best NN methods we have tried, we find that 68\% of the galaxies in the validation set have a photo-z error smaller than {$\sigma$}68 = 0.021 or 0.024. After presenting our results and quality tests, we provide a short guide for users accessing the public data.},
  file = {/home/humphrey/Zotero/storage/KVFUYNM4/Oyaizu et al_2008_A Galaxy Photometric Redshift Catalog for the Sloan Digital Sky Survey Data.pdf},
  journal = {\apj},
  keywords = {catalogs,distance scale,galaxies: distances and redshifts,large-scale structure of universe}
}

@article{oyaizu08b,
  title = {Photometric {{Redshift Error Estimators}}},
  author = {Oyaizu, Hiroaki and Lima, Marcos and Cunha, Carlos E. and Lin, Huan and Frieman, Joshua},
  year = {2008},
  month = dec,
  volume = {689},
  pages = {709--720},
  issn = {0004-637X},
  doi = {10.1086/592591},
  abstract = {Photometric redshift (photo-z) estimates are playing an increasingly important role in extragalactic astronomy and cosmology. Crucial to many photo-z applications is the accurate quantification of photometric redshift errors and their distributions, including identification of likely catastrophic failures in photo-z estimates. We consider several methods of estimating photo-z errors, and propose new training-set based error estimators based on spectroscopic training set data. Using data from the Sloan Digital Sky Survey and simulations of the Dark Energy Survey as examples, we show that this method provides a robust, relatively unbiased estimate of photo-z errors. We show that culling objects with large, accurately estimated photo-z errors from a sample can reduce the incidence of catastrophic photo-z failures.},
  file = {/home/humphrey/Zotero/storage/RU9GDV28/Oyaizu et al_2008_Photometric Redshift Error Estimators.pdf},
  journal = {\apj},
  keywords = {galaxies: distances and redshifts,galaxies: photometry}
}

@article{henderson,
  title = {Advanced {{ACTPol Cryogenic Detector Arrays}} and {{Readout}}},
  author = {Henderson, S. W. and Allison, R. and Austermann, J. and Baildon, T. and Battaglia, N. and Beall, J. A. and Becker, D. and De Bernardis, F. and Bond, J. R. and Calabrese, E. and Choi, S. K. and Coughlin, K. P. and Crowley, K. T. and Datta, R. and Devlin, M. J. and Duff, S. M. and Dunkley, J. and D{\"u}nner, R. and {van Engelen}, A. and Gallardo, P. A. and Grace, E. and Hasselfield, M. and Hills, F. and Hilton, G. C. and Hincks, A. D. and Hlo{\^z}ek, R. and Ho, S. P. and Hubmayr, J. and Huffenberger, K. and Hughes, J. P. and Irwin, K. D. and Koopman, B. J. and Kosowsky, A. B. and Li, D. and McMahon, J. and Munson, C. and Nati, F. and Newburgh, L. and Niemack, M. D. and Niraula, P. and Page, L. A. and Pappas, C. G. and Salatino, M. and Schillaci, A. and Schmitt, B. L. and Sehgal, N. and Sherwin, B. D. and Sievers, J. L. and Simon, S. M. and Spergel, D. N. and Staggs, S. T. and Stevens, J. R. and Thornton, R. and Van Lanen, J. and Vavagiakis, E. M. and Ward, J. T. and Wollack, E. J.},
  year = {2016},
  month = aug,
  volume = {184},
  pages = {772--779},
  issn = {1063-777X0022-2291},
  doi = {10.1007/s10909-016-1575-z},
  abstract = {Advanced ACTPol is a polarization-sensitive upgrade for the 6 m aperture Atacama Cosmology Telescope, adding new frequencies and increasing sensitivity over the previous ACTPol receiver. In 2016, Advanced ACTPol will begin to map approximately half the sky in five frequency bands (28-230 GHz). Its maps of primary and secondary cosmic microwave background anisotropies\textemdash imaged in intensity and polarization at few arcminute-scale resolution\textemdash will enable precision cosmological constraints and also a wide array of cross-correlation science that probes the expansion history of the universe and the growth of structure via gravitational collapse. To accomplish these scientific goals, the Advanced ACTPol receiver will be a significant upgrade to the ACTPol receiver, including four new multichroic arrays of cryogenic, feedhorn-coupled AlMn transition edge sensor polarimeters (fabricated on 150 mm diameter wafers); a system of continuously rotating meta-material silicon half-wave plates; and a new multiplexing readout architecture which uses superconducting quantum interference devices and time division to achieve a 64-row multiplexing factor. Here we present the status and scientific goals of the Advanced ACTPol instrument, emphasizing the design and implementation of the Advanced ACTPol cryogenic detector arrays.},
  file = {/home/humphrey/Zotero/storage/I35KNAKJ/Henderson et al_2016_Advanced ACTPol Cryogenic Detector Arrays and Readout.pdf;/home/humphrey/Zotero/storage/C9A8T5II/abstract.html},
  journal = {	J. Low Temp. Phys.},
  keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics,Astrophysics - Instrumentation and Methods for Astrophysics,Bolometers,Cosmic microwave background,Millimeter-wave,Polarimetry,Superconducting detectors,Transition edge sensors}
}


@article{sptpolinst,
  title = {{{SPTpol}}: An Instrument for {{CMB}} Polarization Measurements with the {{South Pole Telescope}}},
  shorttitle = {{{SPTpol}}},
  author = {Austermann, J. E. and Aird, K. A. and Beall, J. A. and Becker, D. and Bender, A. and Benson, B. A. and Bleem, L. E. and Britton, J. and Carlstrom, J. E. and Chang, C. L. and Chiang, H. C. and Cho, H. -M. and Crawford, T. M. and Crites, A. T. and Datesman, A. and {de Haan}, T. and Dobbs, M. A. and George, E. M. and Halverson, N. W. and Harrington, N. and Henning, J. W. and Hilton, G. C. and Holder, G. P. and Holzapfel, W. L. and Hoover, S. and Huang, N. and Hubmayr, J. and Irwin, K. D. and Keisler, R. and Kennedy, J. and Knox, L. and Lee, A. T. and Leitch, E. and Li, D. and Lueker, M. and Marrone, D. P. and McMahon, J. J. and Mehl, J. and Meyer, S. S. and Montroy, T. E. and Natoli, T. and Nibarger, J. P. and Niemack, M. D. and Novosad, V. and Padin, S. and Pryke, C. and Reichardt, C. L. and Ruhl, J. E. and Saliwanchik, B. R. and Sayre, J. T. and Schaffer, K. K. and Shirokoff, E. and Stark, A. A. and Story, K. and Vanderlinde, K. and Vieira, J. D. and Wang, G. and Williamson, R. and Yefremenko, V. and Yoon, K. W. and Zahn, O.},
  year = {2012},
  month = sep,
  journal = {\procspie},
  volume = {8452},
  pages = {84521E},
  address = {{eprint: arXiv:1210.4970}},
  doi = {10.1117/12.927286},
  abstract = {SPTpol is a dual-frequency polarization-sensitive camera that was deployed on the 10-meter South Pole Telescope in January 2012. SPTpol will measure the polarization anisotropy of the cosmic microwave background (CMB) on angular scales spanning an arcminute to several degrees. The polarization sensitivity of SPTpol will enable a detection of the CMB ``B-mode'' polarization from the detection of the gravitational lensing of the CMB by large scale structure, and a detection or improved upper limit on a primordial signal due to inationary gravity waves. The two measurements can be used to constrain the sum of the neutrino masses and the energy scale of ination. These science goals can be achieved through the polarization sensitivity of the SPTpol camera and careful control of systematics. The SPTpol camera consists of 768 pixels, each containing two transition-edge sensor (TES) bolometers coupled to orthogonal polarizations, and a total of 1536 bolometers. The pixels are sensitive to light in one of two frequency bands centered at 90 and 150 GHz, with 180 pixels at 90 GHz and 588 pixels at 150 GHz. The SPTpol design has several features designed to control polarization systematics, including: singlemoded feedhorns with low cross-polarization, bolometer pairs well-matched to dfference atmospheric signals, an improved ground shield design based on far-sidelobe measurements of the SPT, and a small beam to reduce temperature to polarization leakage. We present an overview of the SPTpol instrument design, project status, and science projections.},
  file = {/home/humphrey/Zotero/storage/J8A5K65X/Austermann et al_2012_SPTpol.pdf;/home/humphrey/Zotero/storage/KPKL7LPB/abstract.html},
  keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics,Astrophysics - Instrumentation and Methods for Astrophysics}
}

@article{thornton,
  title = {The {{Atacama Cosmology Telescope}}: {{The Polarization}}-Sensitive {{ACTPol Instrument}}},
  shorttitle = {The {{Atacama Cosmology Telescope}}},
  author = {Thornton, R. J. and Ade, P. A. R. and Aiola, S. and Angil{\`e}, F. E. and Amiri, M. and Beall, J. A. and Becker, D. T. and Cho, H. -M. and Choi, S. K. and Corlies, P. and Coughlin, K. P. and Datta, R. and Devlin, M. J. and Dicker, S. R. and D{\"u}nner, R. and Fowler, J. W. and Fox, A. E. and Gallardo, P. A. and Gao, J. and Grace, E. and Halpern, M. and Hasselfield, M. and Henderson, S. W. and Hilton, G. C. and Hincks, A. D. and Ho, S. P. and Hubmayr, J. and Irwin, K. D. and Klein, J. and Koopman, B. and Li, Dale and Louis, T. and Lungu, M. and Maurin, L. and McMahon, J. and Munson, C. D. and Naess, S. and Nati, F. and Newburgh, L. and Nibarger, J. and Niemack, M. D. and Niraula, P. and Nolta, M. R. and Page, L. A. and Pappas, C. G. and Schillaci, A. and Schmitt, B. L. and Sehgal, N. and Sievers, J. L. and Simon, S. M. and Staggs, S. T. and Tucker, C. and Uehara, M. and {van Lanen}, J. and Ward, J. T. and Wollack, E. J.},
  year = {2016},
  month = dec,
  volume = {227},
  pages = {21},
  issn = {0067-0049},
  doi = {10.3847/1538-4365/227/2/21},
  abstract = {The Atacama Cosmology Telescope (ACT) makes high angular resolution measurements of anisotropies in the Cosmic Microwave Background (CMB) at millimeter wavelengths. We describe ACTPol, an upgraded receiver for ACT, which uses feedhorn-coupled, polarization-sensitive detector arrays, a 3\textdegree{} field of view, 100 mK cryogenics with continuous cooling, and meta material antireflection coatings. ACTPol comprises three arrays with separate cryogenic optics: two arrays at a central frequency of 148 GHz and one array operating simultaneously at both 97 GHz and 148 GHz. The combined instrument sensitivity, angular resolution, and sky coverage are optimized for measuring angular power spectra, clusters via the thermal Sunyaev-Zel'dovich (SZ) and kinetic SZ signals, and CMB lensing due to large-scale structure. The receiver was commissioned with its first 148 GHz array in 2013, observed with both 148 GHz arrays in 2014, and has recently completed its first full season of operations with the full suite of three arrays. This paper provides an overview of the design and initial performance of the receiver and related systems.},
  file = {/home/humphrey/Zotero/storage/QZ842JHV/Thornton et al_2016_The Atacama Cosmology Telescope.pdf;/home/humphrey/Zotero/storage/AK54RUSD/abstract.html},
  journal = {\apjs},
  keywords = {Astrophysics - Instrumentation and Methods for Astrophysics,cosmic background radiation,instrumentation: polarimeters}
}


@article{Wetzell2021,
    author = {Wetzell, V. and Jeltema, T. E. and Hegland, B. and Everett, S. and Giles, P. A. and Wilkinson, R. and Farahi, A. and Costanzi, M. and Hollowood, D. L. and Upsdell, E. and Saro, A.},
    title = {Velocity Dispersions of Clusters in the Dark Energy Survey Y3 redMaPPer Catalog},
    year = {2021},
    archivePrefix = {arXiv},
    eprint = {2107.07631 [astro-ph]},
    journal = {\mnras}
}


@article{nadler2021,
  title = {Dark {{Matter Constraints}} from a {{Unified Analysis}} of {{Strong Gravitational Lenses}} and {{Milky Way Satellite Galaxies}}},
  author = {Nadler, Ethan O. and Birrer, Simon and Gilman, Daniel and Wechsler, Risa H. and Du, Xiaolong and Benson, Andrew and Nierenberg, Anna M. and Treu, Tommaso},
  year = {2021},
  month = jan,
  abstract = {Joint analyses of small-scale cosmological structure probes are relatively unexplored and promise to advance measurements of microphysical dark matter properties using heterogeneous data. Here, we present a multidimensional analysis of dark matter substructure using strong gravitational lenses and the Milky Way (MW) satellite galaxy population, accounting for degeneracies in model predictions and using covariances in the constraining power of these individual probes for the first time. We simultaneously infer the projected subhalo number density and the half-mode mass describing the suppression of the subhalo mass function in thermal relic warm dark matter (WDM), \$M\_\{\textbackslash mathrm\{hm\}\}\$, using the semi-analytic model \$\textbackslash texttt\{Galacticus\}\$ to connect the subhalo population inferred from MW satellite observations to the strong lensing host halo mass and redshift regime. Combining MW satellite and strong lensing posteriors in this parameter space yields \$M\_\{\textbackslash mathrm\{hm\}\}{$<$}10\^\{7.0\}\textbackslash{} \textbackslash mathrm\{M\}\_\{\textbackslash mathrm\{\textbackslash odot\}\}\$ (WDM particle mass \$m\_\{\textbackslash mathrm\{WDM\}\}{$>$}9.7\textbackslash{} \textbackslash mathrm\{keV\}\$) at \$95\textbackslash\%\$ confidence and disfavors \$M\_\{\textbackslash mathrm\{hm\}\}=10\^\{7.4\}\textbackslash{} \textbackslash mathrm\{M\}\_\{\textbackslash mathrm\{\textbackslash odot\}\}\$ (\$m\_\{\textbackslash mathrm\{WDM\}\}=7.4\textbackslash{} \textbackslash mathrm\{keV\}\$) with a 20:1 marginal likelihood ratio, improving limits on \$m\_\{\textbackslash mathrm\{WDM\}\}\$ set by the two methods independently by \$\textbackslash sim 30\textbackslash\%\$. These results are marginalized over the line-of-sight contribution to the strong lensing signal, the mass of the MW host halo, and the efficiency of subhalo disruption due to baryons, and are robust to differences in the disruption efficiency between the MW and strong lensing regimes at the \$\textbackslash sim 10\textbackslash\%\$ level. This work paves the way for unified analyses of next-generation small-scale structure measurements covering a wide range of scales and redshifts.},
  archiveprefix = {arXiv},
  eprint = {2101.07810},
  eprinttype = {arxiv},
  file = {/home/humphrey/Zotero/storage/W2XFV4ZX/Nadler et al. - 2021 - Dark Matter Constraints from a Unified Analysis of.pdf;/home/humphrey/Zotero/storage/ZVEP9VW5/Nadler et al_2021_Dark Matter Constraints from a Unified Analysis of Strong Gravitational Lenses.pdf;/home/humphrey/Zotero/storage/H767ZNLH/abstract.html;/home/humphrey/Zotero/storage/J6Z23KGJ/2101.html},
  journal = {arXiv:2101.07810 [astro-ph]},
  keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
  primaryclass = {astro-ph}
}

@article{jackodonnell2022,
    author={O'Donnell, J.},
    year = {2022},
    journal={in prep.}
    }
    
    @article{yyzdeblending,
  title = {Crowded {{Cluster Cores}}: {{An Algorithm}} for {{Deblending}} in {{Dark Energy Survey Images}}},
  shorttitle = {Crowded {{Cluster Cores}}},
  author = {Zhang, Yuanyuan and McKay, Timothy A. and Bertin, Emmanuel and Jeltema, Tesla and Miller, Christopher J. and Rykoff, Eli and Song, Jeeseon},
  year = {2015},
  month = nov,
  volume = {127},
  pages = {1183},
  issn = {0004-6280},
  doi = {10.1086/684053},
  abstract = {Deep optical images are often crowded with overlapping objects. This is especially true in the cores of galaxy clusters, where images of dozens of galaxies may lie atop one another. Accurate measurements of cluster properties require deblending algorithms designed to automatically extract a list of individual objects and decide what fraction of the light in each pixel comes from each object. We present new software called the Gradient And INterpolation based deblender (GAIN) as a secondary deblender to improve deblending the images of cluster cores. This software relies on using image intensity gradient and using an image interpolation technique usually used to correct flawed terrestrial digital images. We test this software on Dark Energy Survey coadd images. GAIN helps extracting unbiased photometry measurement for blended sources. It also helps improving detection completeness while introducing only a modest amount of spurious detections. For example, when applied to deep images simulated with high level of deblending difficulties, this software improves detection completeness from 91\% to 97\% for sources above the 10? limiting magnitude at 25.3 mag. We expect this software to be a useful tool for cluster population measurements.},
  file = {/home/humphrey/Zotero/storage/MB5HN3ZI/Zhang et al_2015_Crowded Cluster Cores.pdf},
  journal = {\pasp}
}
    

==> y3_lens_search_objects_table.tex <==
DESJ0002-3332 (A) & 0.527213 & -33.544062 & ($22.67 \pm 0.08$, $21.00 \pm 0.02$, $20.35 \pm 0.02$, $20.02 \pm 0.04$, $19.92 \pm 0.08$) & $0.50 \pm 0.03$ \\
DESJ0002-3332 (B) & 0.527307 & -33.542925 & ($22.45 \pm 0.05$, $21.12 \pm 0.02$, $20.70 \pm 0.02$, $20.45 \pm 0.04$, $20.44 \pm 0.11$) & $0.48 \pm 0.08$ \\
DESJ0002-3332 (1) & 0.525724 & -33.543500 & ($22.12 \pm 0.07$, $21.05 \pm 0.04$, $20.50 \pm 0.04$, $20.27 \pm 0.07$, $20.54 \pm 0.23$) & $0.68 \pm 0.05$ \\
DESJ0002-3332 (2) & 0.526278 & -33.542441 & ($22.57 \pm 0.09$, $21.64 \pm 0.05$, $21.15 \pm 0.05$, $21.12 \pm 0.13$, $21.42 \pm 0.40$) & $0.67 \pm 0.06$ \\
\hline
DESJ0007-4434 (A) & 1.872055 & -44.579515 & ($20.42 \pm 0.01$, $18.73 \pm 0.00$, $18.01 \pm 0.00$, $17.62 \pm 0.01$, $17.45 \pm 0.01$) & $0.51 \pm 0.01$ \\
DESJ0007-4434 (1) & 1.870997 & -44.578933 & ($21.74 \pm 0.01$, $21.01 \pm 0.01$, $20.42 \pm 0.01$, $20.08 \pm 0.01$, $19.95 \pm 0.03$) & $0.73 \pm 0.09$ \\
\hline
DESJ0011-4614 (A) & 2.971390 & -46.239450 & ($20.18 \pm 0.01$, $19.14 \pm 0.00$, $18.46 \pm 0.00$, $18.00 \pm 0.01$, $17.84 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.57 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0011-4614 (1) & 2.970150 & -46.238660 & \ldots & \ldots \\
DESJ0011-4614 (2) & 2.973640 & -46.241360 & \ldots & \ldots \\
\hline
DESJ0014-0057 (A) & 3.725464 & -0.952317 & ($21.14 \pm 0.03$, $19.24 \pm 0.01$, $18.45 \pm 0.01$, $18.04 \pm 0.01$, $17.94 \pm 0.02$) & $0.53 \pm 0.00$ \\
DESJ0014-0057 (1) & 3.728786 & -0.951020 & ($21.25 \pm 0.06$, $20.28 \pm 0.04$, $19.64 \pm 0.03$, $19.41 \pm 0.05$, $19.35 \pm 0.16$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.54 \pm 0.19$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0021-5028 (A) & 5.452849 & -50.476040 & ($20.37 \pm 0.01$, $18.80 \pm 0.00$, $18.26 \pm 0.00$, $17.94 \pm 0.01$, $17.81 \pm 0.02$) & $0.37 \pm 0.02$ \\
DESJ0021-5028 (1) & 5.454124 & -50.475333 & ($21.65 \pm 0.01$, $20.94 \pm 0.01$, $20.63 \pm 0.02$, $20.37 \pm 0.02$, $20.34 \pm 0.08$) & $0.20 \pm 0.06$ \\
\hline
DESJ0025-3139 (A) & 6.292237 & -31.657593 & ($21.38 \pm 0.05$, $19.88 \pm 0.02$, $19.15 \pm 0.02$, $18.81 \pm 0.02$, $18.57 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.56 \pm 0.03$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0025-3139 (1) & 6.291383 & -31.657199 & ($22.09 \pm 0.03$, $21.46 \pm 0.03$, $21.04 \pm 0.03$, $20.78 \pm 0.04$, $20.70 \pm 0.10$) & $0.22 \pm 0.15$ \\
\hline
DESJ0025-4946 (A) & 6.294487 & -49.774042 & ($22.23 \pm 0.06$, $20.66 \pm 0.02$, $19.58 \pm 0.01$, $19.19 \pm 0.02$, $19.04 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.69 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0025-4946 (1) & 6.295470 & -49.774668 & ($22.42 \pm 0.06$, $21.61 \pm 0.04$, $21.03 \pm 0.04$, $20.70 \pm 0.06$, $21.08 \pm 0.24$) & $0.75 \pm 0.06$ \\
\hline
DESJ0026-4825 (A) & 7.049739 & -48.435200 & ($19.37 \pm 0.01$, $17.60 \pm 0.00$, $17.03 \pm 0.00$, $16.71 \pm 0.00$, $16.57 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.38 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0026-4825 (1) & 7.051111 & -48.432314 & ($21.62 \pm 0.02$, $20.57 \pm 0.01$, $20.16 \pm 0.01$, $19.82 \pm 0.02$, $19.67 \pm 0.04$) & $0.45 \pm 0.13$ \\
DESJ0026-4825 (2) & 7.049190 & -48.432200 & \ldots & \ldots \\
\hline
DESJ0030-4507 (A) & 7.663571 & -45.117814 & ($20.88 \pm 0.01$, $19.19 \pm 0.00$, $18.62 \pm 0.00$, $18.28 \pm 0.01$, $18.17 \pm 0.02$) & $0.40 \pm 0.04$ \\
DESJ0030-4507 (1) & 7.661060 & -45.115780 & \ldots & \ldots \\
\hline
DESJ0031-3717 (A) & 7.779623 & -37.292908 & ($22.28 \pm 0.06$, $20.66 \pm 0.02$, $19.56 \pm 0.01$, $19.05 \pm 0.01$, $18.89 \pm 0.03$) & $0.74 \pm 0.03$ \\
DESJ0031-3717 (1) & 7.781746 & -37.293924 & ($22.84 \pm 0.07$, $22.47 \pm 0.07$, $22.18 \pm 0.09$, $21.91 \pm 0.13$, $21.35 \pm 0.25$) & $0.90 \pm 0.35$ \\
DESJ0031-3717 (2) & 7.780348 & -37.292305 & ($23.27 \pm 0.05$, $22.28 \pm 0.03$, $21.67 \pm 0.03$, $21.37 \pm 0.03$, $21.28 \pm 0.10$) & $0.62 \pm 0.11$ \\
DESJ0031-3717 (3) & 7.779335 & -37.291970 & ($22.72 \pm 0.06$, $21.92 \pm 0.04$, $21.51 \pm 0.05$, $21.12 \pm 0.06$, $20.86 \pm 0.16$) & $0.42 \pm 0.12$ \\
\hline
DESJ0032+0100 (A) & 8.073145 & 1.010437 & ($20.08 \pm 0.02$, $18.28 \pm 0.00$, $17.67 \pm 0.00$, $17.33 \pm 0.00$, $17.18 \pm 0.01$)\textsuperscript{\textdagger} & $0.39 \pm 0.00$\textsuperscript{\textdagger} \\
DESJ0032+0100 (1) & 8.072042 & 1.009085 & ($22.30 \pm 0.06$, $21.16 \pm 0.03$, $20.62 \pm 0.03$, $20.41 \pm 0.04$, $20.33 \pm 0.14$)\textsuperscript{\textdagger} & $0.23 \pm 0.06$\textsuperscript{\textdagger} \\
DESJ0032+0100 (2) & 8.071510 & 1.011570 & \ldots & \ldots \\
\hline
DESJ0034+0225 (A) & 8.617365 & 2.422945 & ($20.16 \pm 0.01$, $18.46 \pm 0.00$, $17.88 \pm 0.00$, $17.57 \pm 0.00$, $17.50 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.38 \pm 0.03$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0034+0225 (1) & 8.615521 & 2.426298 & ($23.09 \pm 0.32$, $20.59 \pm 0.04$, $20.27 \pm 0.06$, $20.65 \pm 0.17$, $99.00 \pm 99.00$) & $0.66 \pm 0.71$ \\
DESJ0034+0225 (2) & 8.614283 & 2.422975 & ($21.93 \pm 0.06$, $20.79 \pm 0.03$, $20.45 \pm 0.04$, $20.41 \pm 0.08$, $20.48 \pm 0.24$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.21 \pm 0.18$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0034+0225 (3) & 8.613881 & 2.420758 & ($22.11 \pm 0.05$, $21.66 \pm 0.05$, $21.59 \pm 0.08$, $21.57 \pm 0.17$, $22.62 \pm 1.32$) & $0.72 \pm 0.67$ \\
\hline
DESJ0035-2526 (A) & 8.779998 & -25.449930 & ($22.47 \pm 0.03$, $21.41 \pm 0.01$, $20.49 \pm 0.01$, $20.00 \pm 0.01$, $19.87 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.64 \pm 0.51$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0035-2526 (1) & 8.780002 & -25.450581 & ($20.54 \pm 0.01$, $20.03 \pm 0.01$, $19.85 \pm 0.01$, $19.68 \pm 0.02$, $19.47 \pm 0.05$) & $0.05 \pm 0.05$ \\
\hline
DESJ0038-2155 (A) & 9.716928 & -21.924359 & ($21.15 \pm 0.02$, $19.84 \pm 0.01$, $19.42 \pm 0.01$, $19.15 \pm 0.01$, $18.99 \pm 0.03$) & $0.39 \pm 0.05$ \\
DESJ0038-2155 (1) & 9.717215 & -21.922871 & ($22.42 \pm 0.07$, $21.47 \pm 0.04$, $21.35 \pm 0.06$, $21.13 \pm 0.09$, $21.07 \pm 0.27$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.11 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0038-2155 (2) & 9.715270 & -21.924870 & \ldots & \ldots \\
\hline
DESJ0040-4407 (A) & 10.208260 & -44.130660 & ($19.88 \pm 0.01$, $18.23 \pm 0.00$, $17.66 \pm 0.00$, $17.34 \pm 0.00$, $17.19 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.35 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0040-4407 (1) & 10.211830 & -44.135170 & ($20.81 \pm 0.08$, $18.98 \pm 0.02$, $18.66 \pm 0.03$, $18.46 \pm 0.05$, $19.13 \pm 0.24$) & $0.61 \pm 0.47$ \\
\hline
DESJ0042-6037 (A) & 10.749083 & -60.629126 & ($19.41 \pm 0.01$, $17.83 \pm 0.00$, $17.28 \pm 0.00$, $16.97 \pm 0.00$, $16.87 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.34 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0042-6037 (1) & 10.750000 & -60.631640 & \ldots & \ldots \\
\hline
DESJ0043-6248 (A) & 10.846679 & -62.803256 & ($22.76 \pm 0.08$, $21.02 \pm 0.02$, $20.22 \pm 0.02$, $19.89 \pm 0.03$, $19.67 \pm 0.08$) & $0.58 \pm 0.03$ \\
DESJ0043-6248 (1) & 10.845710 & -62.802480 & \ldots & \ldots \\
\hline
DESJ0043-2037A (A) & 10.852732 & -20.628229 & ($18.56 \pm 0.01$, $17.08 \pm 0.00$, $16.59 \pm 0.00$, $16.30 \pm 0.00$, $16.14 \pm 0.01$) & $0.29 \pm 0.01$ \\
DESJ0043-2037A (1) & 10.859090 & -20.623360 & \ldots & \ldots \\
DESJ0043-2037A (2) & 10.858080 & -20.624290 & \ldots & \ldots \\
DESJ0043-2037A (3) & 10.850970 & -20.623650 & \ldots & \ldots \\
\hline
DESJ0043-2037B (A) & 10.854720 & -20.617010 & ($19.09 \pm 0.00$, $17.60 \pm 0.00$, $17.10 \pm 0.00$, $16.78 \pm 0.00$, $16.63 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.28 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0043-2037B (1) & 10.856070 & -20.621470 & \ldots & \ldots \\
\hline
DESJ0043-3123 (A) & 10.944762 & -31.197894 & ($22.66 \pm 0.06$, $20.71 \pm 0.01$, $19.56 \pm 0.01$, $19.08 \pm 0.01$, $18.92 \pm 0.03$) & $0.70 \pm 0.03$ \\
DESJ0043-3123 (B) & 10.945619 & -31.197946 & ($23.65 \pm 0.08$, $22.05 \pm 0.02$, $20.97 \pm 0.02$, $20.49 \pm 0.02$, $20.35 \pm 0.06$) & $0.74 \pm 0.07$ \\
DESJ0043-3123 (1) & 10.945517 & -31.198745 & ($21.15 \pm 0.02$, $20.50 \pm 0.02$, $20.09 \pm 0.02$, $19.75 \pm 0.03$, $19.66 \pm 0.09$) & $0.46 \pm 0.14$ \\
\hline
DESJ0043-3453 (A) & 10.981430 & -34.887714 & ($23.40 \pm 0.08$, $22.80 \pm 0.06$, $22.17 \pm 0.06$, $21.45 \pm 0.07$, $21.14 \pm 0.14$) & $1.17 \pm 0.09$ \\
DESJ0043-3453 (1) & 10.982428 & -34.888422 & ($20.44 \pm 0.01$, $20.04 \pm 0.01$, $19.83 \pm 0.01$, $19.73 \pm 0.03$, $19.77 \pm 0.08$) & $0.08 \pm 0.04$ \\
\hline
DESJ0044-0448 (A) & 11.021928 & -4.805818 & ($23.12 \pm 0.12$, $21.22 \pm 0.03$, $19.98 \pm 0.01$, $19.44 \pm 0.02$, $19.16 \pm 0.04$) & $0.77 \pm 0.00$ \\
DESJ0044-0448 (1) & 11.022047 & -4.805033 & ($21.85 \pm 0.03$, $21.44 \pm 0.03$, $20.82 \pm 0.03$, $20.54 \pm 0.05$, $20.48 \pm 0.12$) & $0.61 \pm 0.20$ \\
\hline
DESJ0044-0055 (A) & 11.155052 & -0.922286 & ($18.37 \pm 0.00$, $17.13 \pm 0.00$, $16.68 \pm 0.00$, $16.34 \pm 0.00$, $16.22 \pm 0.01$) & $0.20 \pm 0.00$ \\
DESJ0044-0055 (1) & 11.155485 & -0.919887 & ($20.01 \pm 0.02$, $19.00 \pm 0.01$, $18.58 \pm 0.01$, $18.30 \pm 0.02$, $18.12 \pm 0.05$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.07 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0044-0055 (2) & 11.153911 & -0.923678 & ($21.44 \pm 0.02$, $20.24 \pm 0.01$, $19.53 \pm 0.01$, $19.12 \pm 0.01$, $18.96 \pm 0.03$) & $0.53 \pm 0.09$ \\
\hline
DESJ0045-0510 (A) & 11.287328 & -5.178099 & ($18.30 \pm 0.00$, $17.84 \pm 0.00$, $17.57 \pm 0.01$, $17.49 \pm 0.01$, $17.41 \pm 0.02$)\textsuperscript{\textdagger} & $0.12 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0045-0510 (1) & 11.287419 & -5.177041 & ($21.45 \pm 0.01$, $21.08 \pm 0.01$, $20.82 \pm 0.02$, $21.06 \pm 0.05$, $20.83 \pm 0.08$)\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} & $0.18 \pm 0.01$\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} \\
DESJ0045-0510 (2) & 11.287230 & -5.178890 & \ldots & \ldots \\
DESJ0045-0510 (3) & 11.288400 & -5.178450 & \ldots & \ldots \\
\hline
DESJ0045-2013 (A) & 11.441675 & -20.219726 & ($22.26 \pm 0.04$, $21.33 \pm 0.02$, $20.55 \pm 0.02$, $20.25 \pm 0.03$, $20.12 \pm 0.08$) & $0.74 \pm 0.04$ \\
DESJ0045-2013 (1) & 11.441200 & -20.220099 & ($21.14 \pm 0.01$, $20.86 \pm 0.01$, $20.76 \pm 0.02$, $20.76 \pm 0.04$, $20.46 \pm 0.09$) & $0.67 \pm 0.52$ \\
\hline
DESJ0045-0143 (A) & 11.459045 & -1.726783 & ($20.66 \pm 0.01$, $19.65 \pm 0.01$, $19.35 \pm 0.01$, $19.03 \pm 0.01$, $18.90 \pm 0.03$) & $0.44 \pm 0.08$ \\
DESJ0045-0143 (1) & 11.459350 & -1.727090 & \ldots & \ldots \\
\hline
DESJ0045-5159 (A) & 11.493571 & -51.994034 & ($23.83 \pm 0.11$, $22.67 \pm 0.06$, $21.60 \pm 0.04$, $20.72 \pm 0.03$, $20.55 \pm 0.09$) & $1.05 \pm 0.05$ \\
DESJ0045-5159 (1) & 11.493133 & -51.995033 & ($22.88 \pm 0.05$, $22.76 \pm 0.07$, $22.93 \pm 0.14$, $22.67 \pm 0.22$, $24.19 \pm 2.88$) & $0.70 \pm 0.57$ \\
DESJ0045-5159 (2) & 11.492534 & -51.994500 & ($23.68 \pm 0.06$, $23.35 \pm 0.06$, $23.02 \pm 0.08$, $22.78 \pm 0.13$, $22.66 \pm 0.38$) & $0.81 \pm 0.35$ \\
DESJ0045-5159 (3) & 11.491966 & -51.993745 & ($24.31 \pm 0.18$, $23.87 \pm 0.18$, $23.28 \pm 0.18$, $23.20 \pm 0.33$, $21.98 \pm 0.35$) & $0.74 \pm 0.18$ \\
\hline
DESJ0046-0134 (A) & 11.633579 & -1.575573 & ($18.99 \pm 0.00$, $17.65 \pm 0.00$, $17.18 \pm 0.00$, $16.87 \pm 0.00$, $16.72 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.23 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0046-0134 (B) & 11.633691 & -1.577031 & ($19.59 \pm 0.00$, $18.26 \pm 0.00$, $17.82 \pm 0.00$, $17.50 \pm 0.00$, $17.34 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.22 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0046-0134 (1) & 11.632062 & -1.576962 & ($20.60 \pm 0.01$, $19.42 \pm 0.01$, $19.03 \pm 0.01$, $18.74 \pm 0.01$, $18.43 \pm 0.02$) & $0.24 \pm 0.03$ \\
\hline
DESJ0047-5255 (A) & 11.991182 & -52.917494 & ($19.29 \pm 0.00$, $18.99 \pm 0.01$, $18.83 \pm 0.01$, $18.74 \pm 0.01$, $18.74 \pm 0.04$) & $0.08 \pm 0.02$ \\
DESJ0047-5255 (1) & 11.991963 & -52.918490 & ($21.08 \pm 0.01$, $20.95 \pm 0.01$, $20.85 \pm 0.02$, $20.93 \pm 0.05$, $21.20 \pm 0.19$) & $0.93 \pm 0.74$ \\
DESJ0047-5255 (2) & 11.989732 & -52.916998 & ($21.41 \pm 0.01$, $21.44 \pm 0.01$, $21.49 \pm 0.02$, $21.60 \pm 0.04$, $21.57 \pm 0.12$) & $0.77 \pm 0.61$ \\
DESJ0047-5255 (3) & 11.993565 & -52.917326 & ($21.78 \pm 0.02$, $21.80 \pm 0.03$, $21.79 \pm 0.06$, $21.91 \pm 0.13$, $22.80 \pm 0.86$) & $0.69 \pm 0.67$ \\
\hline
DESJ0047-3826 (A) & 11.998543 & -38.445888 & ($18.14 \pm 0.00$, $16.72 \pm 0.00$, $16.24 \pm 0.00$, $15.92 \pm 0.00$, $15.73 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.26 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0047-3826 (1) & 11.997910 & -38.447830 & \ldots & \ldots \\
DESJ0047-3826 (2) & 12.000820 & -38.444320 & \ldots & \ldots \\
\hline
DESJ0048+0311 (A) & 12.113424 & 3.188038 & ($19.83 \pm 0.01$, $18.34 \pm 0.00$, $17.80 \pm 0.00$, $17.49 \pm 0.01$, $17.32 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.36 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0048+0311 (1) & 12.111426 & 3.186980 & ($21.21 \pm 0.02$, $20.88 \pm 0.02$, $20.76 \pm 0.02$, $20.64 \pm 0.04$, $20.37 \pm 0.10$) & $0.59 \pm 0.74$ \\
DESJ0048+0311 (2) & 12.110980 & 3.189020 & \ldots & \ldots \\
\hline
DESJ0057-4848 (A) & 14.403741 & -48.803999 & ($20.68 \pm 0.02$, $19.40 \pm 0.01$, $18.86 \pm 0.01$, $18.55 \pm 0.01$, $18.42 \pm 0.03$) & $0.39 \pm 0.04$ \\
DESJ0057-4848 (1) & 14.404470 & -48.803510 & \ldots & \ldots \\
\hline
DESJ0059-2800 (A) & 14.702191 & -28.011399 & ($18.68 \pm 0.00$, $17.38 \pm 0.00$, $16.94 \pm 0.00$, $16.59 \pm 0.00$, $16.46 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.20 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0059-2800 (1) & 14.701850 & -28.009400 & \ldots & \ldots \\
\hline
DESJ0100-3936 (A) & 15.037439 & -39.615170 & ($18.19 \pm 0.00$, $17.20 \pm 0.00$, $16.82 \pm 0.00$, $16.56 \pm 0.00$, $16.44 \pm 0.01$) & $0.20 \pm 0.00$ \\
DESJ0100-3936 (1) & 15.035380 & -39.614780 & \ldots & \ldots \\
DESJ0100-3936 (2) & 15.039120 & -39.613380 & \ldots & \ldots \\
\hline
DESJ0102-2911 (A) & 15.739573 & -29.189425 & ($18.70 \pm 0.00$, $17.29 \pm 0.00$, $16.81 \pm 0.00$, $16.52 \pm 0.00$, $16.36 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.27 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0102-2911 (1) & 15.739350 & -29.188080 & \ldots & \ldots \\
\hline
DESJ0103-2234 (A) & 15.833679 & -22.569459 & ($18.06 \pm 0.00$, $16.76 \pm 0.00$, $16.32 \pm 0.00$, $16.01 \pm 0.00$, $15.91 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.22 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0103-2234 (1) & 15.835332 & -22.571499 & ($20.78 \pm 0.01$, $19.68 \pm 0.01$, $19.20 \pm 0.01$, $18.89 \pm 0.01$, $18.85 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.22 \pm 0.05$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0103-1821 (A) & 15.844045 & -18.362892 & ($20.55 \pm 0.02$, $18.89 \pm 0.01$, $18.36 \pm 0.01$, $18.06 \pm 0.01$, $17.94 \pm 0.03$) & $0.35 \pm 0.02$ \\
DESJ0103-1821 (1) & 15.843710 & -18.360320 & \ldots & \ldots \\
\hline
DESJ0104-5341 (A) & 16.098370 & -53.699470 & ($21.74 \pm 0.04$, $20.07 \pm 0.01$, $19.11 \pm 0.01$, $18.62 \pm 0.01$, $18.45 \pm 0.03$) & $0.65 \pm 0.02$ \\
DESJ0104-5341 (1) & 16.098250 & -53.700170 & \ldots & \ldots \\
\hline
DESJ0105-3939 (A) & 16.418610 & -39.657320 & ($19.87 \pm 0.01$, $18.26 \pm 0.00$, $17.70 \pm 0.00$, $17.38 \pm 0.01$, $17.26 \pm 0.01$) & $0.38 \pm 0.02$ \\
DESJ0105-3939 (1) & 16.417710 & -39.656780 & \ldots & \ldots \\
\hline
DESJ0105-3520 (A) & 16.469905 & -35.341861 & ($20.77 \pm 0.01$, $19.75 \pm 0.01$, $19.25 \pm 0.01$, $19.03 \pm 0.01$, $18.96 \pm 0.04$) & $0.26 \pm 0.04$ \\
DESJ0105-3520 (1) & 16.470230 & -35.341270 & \ldots & \ldots \\
DESJ0105-3520 (2) & 16.469640 & -35.342190 & \ldots & \ldots \\
DESJ0105-3520 (3) & 16.469210 & -35.341260 & \ldots & \ldots \\
\hline
DESJ0106-3104 (A) & 16.525795 & -31.077393 & ($21.15 \pm 0.05$, $19.65 \pm 0.02$, $18.90 \pm 0.01$, $18.50 \pm 0.02$, $18.14 \pm 0.03$)\textsuperscript{\textdagger} & $0.53 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0106-3104 (1) & 16.526211 & -31.076650 & ($21.37 \pm 0.05$, $20.56 \pm 0.03$, $20.14 \pm 0.03$, $19.68 \pm 0.04$, $19.10 \pm 0.06$)\textsuperscript{\textdagger} & $0.53 \pm 0.02$\textsuperscript{\textdagger} \\
\hline
DESJ0106-3700 (A) & 16.536971 & -37.005421 & ($18.82 \pm 0.00$, $17.38 \pm 0.00$, $16.91 \pm 0.00$, $16.61 \pm 0.00$, $16.45 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.22 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0106-3700 (1) & 16.538310 & -37.006670 & \ldots & \ldots \\
\hline
DESJ0106-5355 (A) & 16.572456 & -53.927213 & ($20.17 \pm 0.01$, $18.34 \pm 0.00$, $17.63 \pm 0.00$, $17.25 \pm 0.00$, $17.01 \pm 0.01$) & $0.48 \pm 0.02$ \\
DESJ0106-5355 (1) & 16.577088 & -53.928236 & ($20.03 \pm 0.01$, $19.84 \pm 0.01$, $19.72 \pm 0.02$, $19.30 \pm 0.03$, $18.96 \pm 0.09$) & $2.50 \pm 0.74$ \\
DESJ0106-5355 (2) & 16.574607 & -53.924750 & ($21.12 \pm 0.03$, $20.66 \pm 0.02$, $20.33 \pm 0.03$, $19.83 \pm 0.04$, $19.00 \pm 0.08$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $1.63 \pm 0.66$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0106-5355 (3) & 16.573272 & -53.930992 & ($20.54 \pm 0.01$, $20.36 \pm 0.01$, $20.22 \pm 0.02$, $19.94 \pm 0.03$, $19.19 \pm 0.05$) & $2.07 \pm 0.84$ \\
DESJ0106-5355 (4) & 16.569838 & -53.925492 & ($20.60 \pm 0.01$, $20.35 \pm 0.01$, $20.15 \pm 0.01$, $19.75 \pm 0.02$, $19.52 \pm 0.07$) & $2.08 \pm 0.80$ \\
DESJ0106-5355 (5) & 16.572410 & -53.924220 & \ldots & \ldots \\
DESJ0106-5355 (6) & 16.569710 & -53.930800 & \ldots & \ldots \\
\hline
DESJ0107-3128 (A) & 16.770516 & -31.478048 & ($22.02 \pm 0.03$, $20.47 \pm 0.01$, $19.32 \pm 0.01$, $18.73 \pm 0.01$, $18.45 \pm 0.02$) & $0.78 \pm 0.02$ \\
DESJ0107-3128 (1) & 16.771475 & -31.476672 & ($21.69 \pm 0.03$, $21.12 \pm 0.03$, $20.82 \pm 0.04$, $20.68 \pm 0.07$, $20.77 \pm 0.21$) & $0.26 \pm 0.05$ \\
DESJ0107-3128 (2) & 16.772050 & -31.477959 & ($21.96 \pm 0.03$, $21.32 \pm 0.02$, $21.15 \pm 0.04$, $20.87 \pm 0.06$, $20.68 \pm 0.14$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.34 \pm 0.10$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0107-3128 (3) & 16.771480 & -31.479279 & ($22.06 \pm 0.04$, $21.47 \pm 0.03$, $21.30 \pm 0.05$, $20.90 \pm 0.07$, $20.44 \pm 0.13$) & $0.35 \pm 0.14$ \\
DESJ0107-3128 (4) & 16.769110 & -31.478160 & \ldots & \ldots \\
\hline
DESJ0109-3335 (A) & 17.469500 & -33.592600 & ($20.21 \pm 0.02$, $18.44 \pm 0.00$, $17.75 \pm 0.00$, $17.36 \pm 0.00$, $17.24 \pm 0.01$) & $0.48 \pm 0.01$ \\
DESJ0109-3335 (1) & 17.472340 & -33.592920 & \ldots & \ldots \\
\hline
\hline
DESJ0115-3520 (A) & 18.920163 & -35.338748 & ($20.65 \pm 0.01$, $19.40 \pm 0.01$, $18.69 \pm 0.01$, $18.37 \pm 0.01$, $18.27 \pm 0.02$) & $0.63 \pm 0.07$ \\
DESJ0115-3520 (1) & 18.921480 & -35.339626 & ($22.78 \pm 0.03$, $22.03 \pm 0.02$, $21.59 \pm 0.03$, $21.39 \pm 0.04$, $21.45 \pm 0.13$) & $0.62 \pm 0.42$ \\
\hline
DESJ0128-2905 (A) & 22.143197 & -29.092019 & ($20.57 \pm 0.00$, $19.08 \pm 0.00$, $18.57 \pm 0.00$, $18.26 \pm 0.00$, $18.14 \pm 0.01$) & $0.28 \pm 0.01$ \\
DESJ0128-2905 (1) & 22.141762 & -29.091288 & ($20.86 \pm 0.03$, $19.31 \pm 0.01$, $18.77 \pm 0.01$, $18.40 \pm 0.02$, $18.13 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.18 \pm 0.06$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0128-2957 (A) & 22.212328 & -29.960199 & ($21.57 \pm 0.04$, $20.24 \pm 0.02$, $19.31 \pm 0.01$, $18.93 \pm 0.02$, $18.65 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.65 \pm 0.03$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0128-2957 (1) & 22.212860 & -29.959450 & \ldots & \ldots \\
DESJ0128-2957 (2) & 22.213660 & -29.960320 & \ldots & \ldots \\
\hline
DESJ0129-1641 (A) & 22.294377 & -16.684065 & ($22.89 \pm 0.05$, $21.88 \pm 0.03$, $20.84 \pm 0.02$, $20.05 \pm 0.02$, $19.80 \pm 0.05$) & $1.05 \pm 0.05$ \\
DESJ0129-1641 (1) & 22.293878 & -16.683333 & ($20.86 \pm 0.01$, $20.66 \pm 0.01$, $20.57 \pm 0.02$, $20.42 \pm 0.03$, $20.61 \pm 0.14$) & $0.89 \pm 0.64$ \\
\hline
DESJ0130-3744 (A) & 22.512071 & -37.749394 & ($21.28 \pm 0.02$, $19.51 \pm 0.01$, $18.53 \pm 0.00$, $18.08 \pm 0.01$, $17.92 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.62 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0130-3744 (1) & 22.512726 & -37.750775 & ($21.99 \pm 0.04$, $21.16 \pm 0.03$, $20.66 \pm 0.03$, $20.36 \pm 0.05$, $20.22 \pm 0.14$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.63 \pm 0.21$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0130-3744 (2) & 22.513552 & -37.749210 & ($22.08 \pm 0.03$, $21.28 \pm 0.02$, $20.71 \pm 0.02$, $20.36 \pm 0.03$, $20.27 \pm 0.10$) & $0.73 \pm 0.17$ \\
DESJ0130-3744 (3) & 22.510611 & -37.750749 & ($22.39 \pm 0.02$, $21.80 \pm 0.02$, $21.40 \pm 0.02$, $21.12 \pm 0.04$, $21.08 \pm 0.12$) & $0.61 \pm 0.23$ \\
\hline
DESJ0131-1336 (A) & 22.968889 & -13.611217 & ($17.59 \pm 0.00$, $99.00 \pm 99.00$, $99.00 \pm 99.00$, $15.63 \pm 0.00$, $15.47 \pm 0.01$)\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} & $4.41 \pm 108.20$\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} \\
DESJ0131-1336 (1) & 22.963933 & -13.607115 & ($20.89 \pm 0.03$, $99.00 \pm 99.00$, $99.00 \pm 99.00$, $19.34 \pm 0.05$, $19.37 \pm 0.13$)\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} & $4.41 \pm 108.20$\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0133-1650 (A) & 23.423949 & -16.839027 & ($21.95 \pm 0.03$, $20.51 \pm 0.01$, $19.59 \pm 0.01$, $19.20 \pm 0.02$, $19.03 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.66 \pm 0.07$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0133-1650 (1) & 23.423160 & -16.840420 & \ldots & \ldots \\
\hline
DESJ0133-6434 (A) & 23.477735 & -64.570279 & ($19.25 \pm 0.01$, $17.79 \pm 0.00$, $17.27 \pm 0.00$, $16.98 \pm 0.00$, $16.86 \pm 0.01$)\textsuperscript{\textdagger} & $0.31 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0133-6434 (1) & 23.475159 & -64.571037 & ($20.36 \pm 0.02$, $19.59 \pm 0.01$, $19.25 \pm 0.02$, $19.09 \pm 0.03$, $19.00 \pm 0.08$)\textsuperscript{\textdagger} & $0.10 \pm 0.02$\textsuperscript{\textdagger} \\
DESJ0133-6434 (2) & 23.475774 & -64.569528 & ($20.44 \pm 0.01$, $19.88 \pm 0.01$, $19.65 \pm 0.01$, $19.42 \pm 0.01$, $19.29 \pm 0.04$)\textsuperscript{\textdagger} & $0.04 \pm 0.01$\textsuperscript{\textdagger} \\
\hline
DESJ0134+0433 (A) & 23.676554 & 4.563913 & ($20.74 \pm 0.04$, $19.14 \pm 0.01$, $18.33 \pm 0.01$, $17.90 \pm 0.01$, $17.82 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.55 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0134+0433 (1) & 23.675207 & 4.563759 & ($21.59 \pm 0.04$, $21.01 \pm 0.03$, $20.66 \pm 0.03$, $20.35 \pm 0.04$, $19.92 \pm 0.10$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.62 \pm 0.25$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0135-2328 (A) & 23.800351 & -23.473269 & ($18.26 \pm 0.00$, $17.03 \pm 0.00$, $16.61 \pm 0.00$, $16.32 \pm 0.00$, $16.28 \pm 0.01$) & $0.22 \pm 0.00$ \\
DESJ0135-2328 (1) & 23.798500 & -23.472750 & \ldots & \ldots \\
\hline
DESJ0135-2033 (A) & 23.928307 & -20.559859 & ($20.99 \pm 0.03$, $19.55 \pm 0.01$, $18.62 \pm 0.01$, $18.23 \pm 0.01$, $18.04 \pm 0.04$)\textsuperscript{\textdagger} & $0.61 \pm 0.02$\textsuperscript{\textdagger} \\
DESJ0135-2033 (1) & 23.927347 & -20.558628 & ($22.21 \pm 0.08$, $21.46 \pm 0.04$, $20.91 \pm 0.05$, $20.51 \pm 0.09$, $20.24 \pm 0.20$)\textsuperscript{\textdagger} & $0.78 \pm 0.17$\textsuperscript{\textdagger} \\
DESJ0135-2033 (2) & 23.927065 & -20.559951 & ($22.28 \pm 0.02$, $22.02 \pm 0.02$, $21.66 \pm 0.03$, $21.63 \pm 0.07$, $21.26 \pm 0.14$)\textsuperscript{\textdagger} & $0.14 \pm 0.12$\textsuperscript{\textdagger} \\
DESJ0135-2033 (3) & 23.928000 & -20.561091 & ($22.24 \pm 0.06$, $22.06 \pm 0.06$, $21.53 \pm 0.06$, $21.43 \pm 0.13$, $20.57 \pm 0.22$)\textsuperscript{\textdagger} & $0.71 \pm 0.13$\textsuperscript{\textdagger} \\
\hline
DESJ0137-1034 (A) & 24.293998 & -10.572778 & ($21.04 \pm 0.04$, $19.13 \pm 0.01$, $18.04 \pm 0.01$, $17.58 \pm 0.01$, $17.45 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.66 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0137-1034 (1) & 24.291438 & -10.575724 & ($21.88 \pm 0.08$, $21.16 \pm 0.05$, $20.34 \pm 0.04$, $20.01 \pm 0.06$, $20.12 \pm 0.22$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $1.19 \pm 0.14$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0138-2155 (A) & 24.515739 & -21.925421 & ($18.42 \pm 0.00$, $17.00 \pm 0.00$, $16.48 \pm 0.00$, $16.12 \pm 0.00$, $16.05 \pm 0.01$) & $0.16 \pm 0.01$ \\
DESJ0138-2155 (1) & 24.515951 & -21.930162 & ($21.43 \pm 0.06$, $19.78 \pm 0.02$, $19.34 \pm 0.02$, $18.77 \pm 0.03$, $18.63 \pm 0.08$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.58 \pm 0.12$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0138-2155 (2) & 24.513301 & -21.929919 & ($22.02 \pm 0.05$, $20.49 \pm 0.02$, $19.93 \pm 0.02$, $19.29 \pm 0.02$, $18.95 \pm 0.05$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.26 \pm 0.22$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0138-2155 (3) & 24.509989 & -21.926020 & ($22.11 \pm 0.08$, $20.76 \pm 0.03$, $20.27 \pm 0.04$, $19.58 \pm 0.04$, $19.75 \pm 0.14$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.96 \pm 0.14$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0138-2844 (A) & 24.595731 & -28.735568 & ($20.46 \pm 0.01$, $19.07 \pm 0.00$, $18.53 \pm 0.00$, $18.20 \pm 0.01$, $17.96 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.35 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0138-2844 (1) & 24.594750 & -28.735090 & \ldots & \ldots \\
\hline
DESJ0143-0850 (A) & 25.862212 & -8.839277 & ($21.35 \pm 0.03$, $20.33 \pm 0.02$, $19.50 \pm 0.01$, $19.11 \pm 0.02$, $18.93 \pm 0.05$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.72 \pm 0.05$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0143-0850 (1) & 25.861630 & -8.838780 & \ldots & \ldots \\
DESJ0143-0850 (2) & 25.861620 & -8.839290 & \ldots & \ldots \\
DESJ0143-0850 (3) & 25.861950 & -8.839940 & \ldots & \ldots \\
\hline
DESJ0143-2617 (A) & 25.939008 & -26.294625 & ($19.77 \pm 0.01$, $18.17 \pm 0.00$, $17.64 \pm 0.00$, $17.32 \pm 0.00$, $17.20 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.33 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0143-2617 (1) & 25.938090 & -26.296010 & \ldots & \ldots \\
\hline
DESJ0144-2213 (A) & 26.168409 & -22.229448 & ($18.49 \pm 0.00$, $16.99 \pm 0.00$, $16.51 \pm 0.00$, $16.20 \pm 0.00$, $16.06 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.28 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0144-2213 (1) & 26.171953 & -22.229090 & ($20.55 \pm 0.03$, $19.24 \pm 0.01$, $18.73 \pm 0.01$, $18.38 \pm 0.02$, $18.33 \pm 0.07$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.30 \pm 0.10$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0145-0455 (A) & 26.267927 & -4.930875 & ($20.37 \pm 0.02$, $19.54 \pm 0.01$, $18.86 \pm 0.01$, $18.50 \pm 0.01$, $18.40 \pm 0.03$) & $0.53 \pm 0.18$ \\
DESJ0145-0455 (1) & 26.268430 & -4.930460 & \ldots & \ldots \\
\hline
DESJ0145+0137 (A) & 26.303602 & 1.619489 & ($17.70 \pm 0.00$, $16.38 \pm 0.00$, $15.92 \pm 0.00$, $15.61 \pm 0.00$, $15.42 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.23 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0145+0137 (1) & 26.306350 & 1.620100 & \ldots & \ldots \\
\hline
DESJ0145-3541 (A) & 26.444990 & -35.690953 & ($20.80 \pm 0.02$, $19.33 \pm 0.01$, $18.66 \pm 0.01$, $18.27 \pm 0.01$, $18.09 \pm 0.02$) & $0.51 \pm 0.05$ \\
DESJ0145-3541 (1) & 26.445320 & -35.690084 & ($21.00 \pm 0.01$, $20.62 \pm 0.01$, $20.34 \pm 0.02$, $20.06 \pm 0.02$, $19.83 \pm 0.05$) & $0.61 \pm 0.17$ \\
\hline
DESJ0146-0929 (A) & 26.733460 & -9.497800 & ($19.90 \pm 0.01$, $18.05 \pm 0.00$, $17.41 \pm 0.00$, $17.04 \pm 0.00$, $16.91 \pm 0.01$) & $0.45 \pm 0.00$ \\
DESJ0146-0929 (1) & 26.736240 & -9.496680 & ($22.01 \pm 0.08$, $20.88 \pm 0.04$, $20.40 \pm 0.04$, $20.15 \pm 0.06$, $20.06 \pm 0.20$) & $0.91 \pm 0.18$ \\
DESJ0146-0929 (2) & 26.730610 & -9.495340 & ($21.51 \pm 0.05$, $20.47 \pm 0.03$, $19.94 \pm 0.03$, $19.65 \pm 0.04$, $19.52 \pm 0.13$) & $0.40 \pm 0.13$ \\
DESJ0146-0929 (3) & 26.732530 & -9.501020 & \ldots & \ldots \\
\hline
DESJ0149-3825 (A) & 27.359280 & -38.425420 & ($20.20 \pm 0.01$, $18.51 \pm 0.00$, $17.94 \pm 0.00$, $17.63 \pm 0.00$, $17.48 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.36 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0149-3825 (1) & 27.356830 & -38.423640 & \ldots & \ldots \\
\hline
DESJ0151-3544A (A) & 27.817714 & -35.737422 & ($21.66 \pm 0.04$, $19.97 \pm 0.01$, $19.16 \pm 0.01$, $18.73 \pm 0.01$, $18.65 \pm 0.03$)\textsuperscript{\textdagger} & $0.54 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0151-3544A (1) & 27.819883 & -35.738439 & ($22.00 \pm 0.07$, $21.40 \pm 0.06$, $21.05 \pm 0.07$, $20.91 \pm 0.10$, $20.64 \pm 0.25$)\textsuperscript{\textdagger} & $0.19 \pm 0.04$\textsuperscript{\textdagger} \\
\hline
DESJ0151-3544B (A) & 27.817750 & -35.737460 & ($20.94 \pm 0.02$, $19.53 \pm 0.01$, $18.79 \pm 0.01$, $18.39 \pm 0.01$, $18.27 \pm 0.03$) & $0.53 \pm 0.01$ \\
DESJ0151-3544B (B) & 27.820720 & -35.740740 & ($21.85 \pm 0.03$, $20.26 \pm 0.01$, $19.52 \pm 0.01$, $19.15 \pm 0.01$, $18.97 \pm 0.04$) & $0.55 \pm 0.03$ \\
DESJ0151-3544B (1) & 27.823619 & -35.744074 & ($21.45 \pm 0.05$, $20.45 \pm 0.02$, $19.92 \pm 0.03$, $19.55 \pm 0.03$, $19.35 \pm 0.10$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.58 \pm 0.13$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0152-2853 (A) & 28.143580 & -28.893791 & ($20.50 \pm 0.01$, $18.72 \pm 0.00$, $18.14 \pm 0.00$, $17.80 \pm 0.01$, $17.74 \pm 0.02$) & $0.42 \pm 0.00$ \\
DESJ0152-2853 (1) & 28.146420 & -28.897449 & ($21.34 \pm 0.02$, $20.82 \pm 0.02$, $20.59 \pm 0.02$, $20.29 \pm 0.03$, $20.02 \pm 0.09$) & $0.71 \pm 0.22$ \\
DESJ0152-2853 (2) & 28.143740 & -28.898490 & \ldots & \ldots \\
\hline
DESJ0154-2324 (A) & 28.609636 & -23.406691 & ($24.02 \pm 0.21$, $21.65 \pm 0.03$, $20.49 \pm 0.02$, $20.00 \pm 0.02$, $19.69 \pm 0.07$) & $0.78 \pm 0.03$ \\
DESJ0154-2324 (1) & 28.610544 & -23.407159 & ($22.36 \pm 0.04$, $21.93 \pm 0.03$, $21.56 \pm 0.04$, $21.57 \pm 0.08$, $22.76 \pm 0.95$) & $0.45 \pm 0.71$ \\
DESJ0154-2324 (2) & 28.610700 & -23.406334 & ($22.28 \pm 0.03$, $22.02 \pm 0.03$, $21.77 \pm 0.05$, $21.94 \pm 0.10$, $21.61 \pm 0.30$) & $1.10 \pm 0.61$ \\
\hline
DESJ0158-0040 (A) & 29.603200 & -0.666490 & ($21.30 \pm 0.05$, $19.92 \pm 0.03$, $19.14 \pm 0.02$, $18.64 \pm 0.02$, $18.60 \pm 0.08$)\textsuperscript{\textdagger} & $0.59 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0158-0040 (B) & 29.603180 & -0.666940 & ($23.27 \pm 0.08$, $21.61 \pm 0.04$, $20.79 \pm 0.03$, $20.36 \pm 0.03$, $20.16 \pm 0.08$)\textsuperscript{\textdagger} & $0.61 \pm 0.03$\textsuperscript{\textdagger} \\
DESJ0158-0040 (1) & 29.602480 & -0.666720 & \ldots & \ldots \\
DESJ0158-0040 (2) & 29.603150 & -0.667690 & \ldots & \ldots \\
\hline
DESJ0159-3413 (A) & 29.766620 & -34.217860 & ($19.73 \pm 0.01$, $17.95 \pm 0.00$, $17.38 \pm 0.00$, $17.02 \pm 0.01$, $16.89 \pm 0.01$)\textsuperscript{\textdagger} & $0.36 \pm 0.00$\textsuperscript{\textdagger} \\
DESJ0159-3413 (1) & 29.769510 & -34.216520 & ($23.00 \pm 0.08$, $21.68 \pm 0.05$, $21.20 \pm 0.05$, $20.72 \pm 0.05$, $20.73 \pm 0.12$)\textsuperscript{\textdagger} & $0.61 \pm 0.06$\textsuperscript{\textdagger} \\
DESJ0159-3413 (2) & 29.770020 & -34.217800 & \ldots & \ldots \\
DESJ0159-3413 (3) & 29.770150 & -34.218930 & \ldots & \ldots \\
\hline
DESJ0159-3413ALT (A) & 29.766620 & -34.217860 & ($19.73 \pm 0.01$, $17.95 \pm 0.00$, $17.38 \pm 0.00$, $17.02 \pm 0.01$, $16.89 \pm 0.01$)\textsuperscript{\textdagger} & $0.36 \pm 0.00$\textsuperscript{\textdagger} \\
DESJ0159-3413ALT (1) & 29.765970 & -34.220770 & ($23.92 \pm 0.11$, $23.44 \pm 0.15$, $23.10 \pm 0.17$, $23.24 \pm 0.32$, $23.95 \pm 1.50$)\textsuperscript{\textdagger} & $0.98 \pm 0.28$\textsuperscript{\textdagger} \\
DESJ0159-3413ALT (2) & 29.764640 & -34.217640 & \ldots & \ldots \\
DESJ0159-3413ALT (3) & 29.765300 & -34.216040 & \ldots & \ldots \\
\hline
DESJ0200+0127 (A) & 30.240176 & 1.463631 & ($21.47 \pm 0.04$, $20.48 \pm 0.02$, $19.68 \pm 0.02$, $19.44 \pm 0.03$, $19.20 \pm 0.07$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.65 \pm 0.05$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0200+0127 (1) & 30.240327 & 1.464728 & ($21.62 \pm 0.04$, $20.69 \pm 0.02$, $20.25 \pm 0.03$, $20.08 \pm 0.04$, $19.81 \pm 0.11$) & $0.25 \pm 0.04$ \\
\hline
DESJ0203-2338 (A) & 30.766741 & -23.634049 & ($20.81 \pm 0.02$, $19.53 \pm 0.01$, $18.70 \pm 0.01$, $18.30 \pm 0.01$, $18.23 \pm 0.03$) & $0.61 \pm 0.01$ \\
DESJ0203-2338 (1) & 30.767096 & -23.633132 & ($22.62 \pm 0.04$, $22.18 \pm 0.04$, $21.97 \pm 0.05$, $21.78 \pm 0.08$, $22.50 \pm 0.57$) & $0.48 \pm 0.70$ \\
DESJ0203-2338 (2) & 30.765960 & -23.633120 & \ldots & \ldots \\
\hline
DESJ0203-2017 (A) & 30.793572 & -20.291461 & ($23.05 \pm 0.10$, $21.34 \pm 0.03$, $20.77 \pm 0.03$, $20.35 \pm 0.04$, $20.07 \pm 0.14$) & $0.44 \pm 0.04$ \\
DESJ0203-2017 (1) & 30.793970 & -20.293070 & \ldots & \ldots \\
\hline
DESJ0203-3104 (A) & 30.915258 & -31.082313 & ($21.33 \pm 0.02$, $20.04 \pm 0.01$, $19.47 \pm 0.01$, $19.10 \pm 0.01$, $19.05 \pm 0.03$) & $0.46 \pm 0.07$ \\
DESJ0203-3104 (1) & 30.914810 & -31.082750 & \ldots & \ldots \\
DESJ0203-3104 (2) & 30.915810 & -31.081750 & \ldots & \ldots \\
\hline
DESJ0205-3539 (A) & 31.358770 & -35.663180 & ($19.72 \pm 0.01$, $18.15 \pm 0.00$, $17.61 \pm 0.00$, $17.28 \pm 0.00$, $17.16 \pm 0.01$) & $0.34 \pm 0.01$ \\
DESJ0205-3539 (1) & 31.357750 & -35.662750 & \ldots & \ldots \\
\hline
DESJ0205-1935 (A) & 31.436178 & -19.594480 & ($23.88 \pm 0.18$, $22.14 \pm 0.05$, $21.14 \pm 0.03$, $20.73 \pm 0.04$, $20.67 \pm 0.15$) & $0.63 \pm 0.03$ \\
DESJ0205-1935 (1) & 31.436754 & -19.595545 & ($22.45 \pm 0.07$, $22.21 \pm 0.07$, $21.69 \pm 0.09$, $21.61 \pm 0.15$, $21.94 \pm 0.75$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.45 \pm 0.85$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0206+0258 (A) & 31.522325 & 2.980347 & ($20.88 \pm 0.02$, $19.41 \pm 0.01$, $18.80 \pm 0.01$, $18.39 \pm 0.01$, $18.28 \pm 0.03$) & $0.46 \pm 0.00$ \\
DESJ0206+0258 (1) & 31.521860 & 2.981400 & \ldots & \ldots \\
\hline
DESJ0206-0114 (A) & 31.556124 & -1.238199 & ($20.56 \pm 0.02$, $19.85 \pm 0.01$, $19.16 \pm 0.01$, $18.68 \pm 0.01$, $18.52 \pm 0.04$) & $0.48 \pm 0.25$ \\
DESJ0206-0114 (1) & 31.556570 & -1.238460 & \ldots & \ldots \\
DESJ0206-0114 (2) & 31.555460 & -1.238470 & \ldots & \ldots \\
\hline
DESJ0207-2726 (A) & 31.777780 & -27.445810 & ($18.79 \pm 0.00$, $17.78 \pm 0.00$, $17.33 \pm 0.00$, $17.04 \pm 0.00$, $16.86 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.27 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0207-2726 (1) & 31.777470 & -27.444450 & \ldots & \ldots \\
DESJ0207-2726 (2) & 31.778750 & -27.446250 & \ldots & \ldots \\
DESJ0207-2726 (3) & 31.776500 & -27.446370 & \ldots & \ldots \\
\hline
DESJ0209+0222 (A) & 32.407416 & 2.382447 & ($20.55 \pm 0.02$, $18.74 \pm 0.01$, $18.16 \pm 0.01$, $17.82 \pm 0.01$, $17.74 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.41 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0209+0222 (1) & 32.405900 & 2.383970 & \ldots & \ldots \\
\hline
DESJ0209-3547 (A) & 32.476490 & -35.799028 & ($19.85 \pm 0.01$, $18.41 \pm 0.00$, $17.90 \pm 0.00$, $17.59 \pm 0.00$, $17.45 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.30 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0209-3547 (B) & 32.477616 & -35.799240 & ($20.86 \pm 0.01$, $19.31 \pm 0.00$, $18.79 \pm 0.00$, $18.48 \pm 0.00$, $18.35 \pm 0.01$) & $0.35 \pm 0.03$ \\
DESJ0209-3547 (1) & 32.477590 & -35.800410 & \ldots & \ldots \\
\hline
DESJ0212-2842 (A) & 33.114415 & -28.716135 & ($18.36 \pm 0.00$, $17.05 \pm 0.00$, $16.61 \pm 0.00$, $16.31 \pm 0.00$, $16.15 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.26 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0212-2842 (1) & 33.115890 & -28.717580 & \ldots & \ldots \\
DESJ0212-2842 (2) & 33.116300 & -28.716030 & \ldots & \ldots \\
\hline
DESJ0214-0535 (A) & 33.533852 & -5.592691 & ($21.10 \pm 0.01$, $19.32 \pm 0.00$, $18.69 \pm 0.00$, $18.31 \pm 0.00$, $18.17 \pm 0.01$) & $0.45 \pm 0.00$ \\
DESJ0214-0535 (B) & 33.533564 & -5.591992 & ($20.64 \pm 0.01$, $19.18 \pm 0.00$, $18.58 \pm 0.00$, $18.24 \pm 0.00$, $18.09 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.45 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0214-0535 (1) & 33.533510 & -5.594470 & \ldots & \ldots \\
DESJ0214-0535 (2) & 33.532830 & -5.590690 & \ldots & \ldots \\
\hline
DESJ0214-0206 (A) & 33.533346 & -2.107934 & ($20.98 \pm 0.02$, $20.02 \pm 0.01$, $19.21 \pm 0.01$, $18.82 \pm 0.01$, $18.70 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.67 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0214-0206 (1) & 33.534204 & -2.108192 & ($23.08 \pm 0.05$, $22.43 \pm 0.04$, $22.03 \pm 0.05$, $21.63 \pm 0.06$, $21.35 \pm 0.15$) & $0.79 \pm 0.34$ \\
DESJ0214-0206 (2) & 33.533860 & -2.108760 & \ldots & \ldots \\
DESJ0214-0206 (3) & 33.532710 & -2.108330 & \ldots & \ldots \\
\hline
DESJ0214-4207 (A) & 33.695592 & -42.117894 & ($19.59 \pm 0.01$, $18.26 \pm 0.00$, $17.78 \pm 0.00$, $17.51 \pm 0.01$, $17.34 \pm 0.02$) & $0.27 \pm 0.02$ \\
DESJ0214-4207 (1) & 33.695150 & -42.118490 & \ldots & \ldots \\
\hline
DESJ0218-3142 (A) & 34.582248 & -31.704951 & ($18.51 \pm 0.01$, $17.03 \pm 0.00$, $16.55 \pm 0.00$, $16.24 \pm 0.00$, $16.12 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.28 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0218-3142 (1) & 34.581075 & -31.702811 & ($21.10 \pm 0.02$, $19.53 \pm 0.01$, $18.87 \pm 0.01$, $18.35 \pm 0.01$, $18.16 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.23 \pm 0.06$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0219-4427 (A) & 34.792757 & -44.454265 & ($18.27 \pm 0.00$, $17.26 \pm 0.00$, $16.82 \pm 0.00$, $16.56 \pm 0.00$, $16.41 \pm 0.01$) & $0.21 \pm 0.01$ \\
DESJ0219-4427 (1) & 34.793940 & -44.454930 & \ldots & \ldots \\
\hline
DESJ0219+0247 (A) & 34.972893 & 2.785353 & ($18.90 \pm 0.00$, $17.44 \pm 0.00$, $16.95 \pm 0.00$, $16.62 \pm 0.00$, $16.46 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.25 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0219+0247 (1) & 34.968430 & 2.783700 & \ldots & \ldots \\
\hline
DESJ0220-3833 (A) & 35.240320 & -38.550920 & ($19.69 \pm 0.01$, $18.15 \pm 0.00$, $17.58 \pm 0.00$, $17.24 \pm 0.00$, $17.07 \pm 0.01$)\textsuperscript{\textdagger} & $0.33 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0220-3833 (1) & 35.239950 & -38.553670 & ($21.95 \pm 0.04$, $20.85 \pm 0.03$, $20.26 \pm 0.02$, $19.86 \pm 0.03$, $19.46 \pm 0.06$)\textsuperscript{\textdagger} & $0.55 \pm 0.06$\textsuperscript{\textdagger} \\
DESJ0220-3833 (2) & 35.240310 & -38.549440 & \ldots & \ldots \\
DESJ0220-3833 (3) & 35.238010 & -38.553050 & \ldots & \ldots \\
DESJ0220-3833 (4) & 35.243310 & -38.552710 & \ldots & \ldots \\
\hline
DESJ0225-4200 (A) & 36.353230 & -42.015556 & ($18.03 \pm 0.00$, $16.73 \pm 0.00$, $16.29 \pm 0.00$, $15.94 \pm 0.00$, $15.74 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.22 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0225-4200 (1) & 36.356460 & -42.013810 & \ldots & \ldots \\
\hline
DESJ0227-4516 (A) & 36.791070 & -45.275330 & ($20.02 \pm 0.02$, $18.43 \pm 0.01$, $17.82 \pm 0.01$, $17.44 \pm 0.01$, $17.25 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.44 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0227-4516 (1) & 36.792460 & -45.274810 & \ldots & \ldots \\
\hline
DESJ0229-3110 (A) & 37.484438 & -31.172977 & ($21.36 \pm 0.03$, $20.22 \pm 0.01$, $19.65 \pm 0.01$, $19.31 \pm 0.02$, $19.14 \pm 0.05$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.49 \pm 0.05$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0229-3110 (B) & 37.483730 & -31.172969 & ($22.41 \pm 0.04$, $20.73 \pm 0.01$, $20.02 \pm 0.01$, $19.69 \pm 0.02$, $19.63 \pm 0.05$) & $0.48 \pm 0.05$ \\
DESJ0229-3110 (1) & 37.485220 & -31.174260 & \ldots & \ldots \\
\hline
DESJ0230-2702 (A) & 37.702677 & -27.041590 & ($20.51 \pm 0.02$, $18.86 \pm 0.01$, $18.30 \pm 0.01$, $17.95 \pm 0.01$, $17.79 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.33 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0230-2702 (1) & 37.703490 & -27.039960 & ($21.45 \pm 0.05$, $20.09 \pm 0.02$, $19.55 \pm 0.02$, $19.41 \pm 0.04$, $19.02 \pm 0.08$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.49 \pm 0.29$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
\hline
DESJ0237-3017 (A) & 39.348430 & -30.292090 & ($21.32 \pm 0.02$, $19.60 \pm 0.01$, $18.78 \pm 0.00$, $18.36 \pm 0.01$, $18.25 \pm 0.02$) & $0.55 \pm 0.02$ \\
DESJ0237-3017 (B) & 39.347468 & -30.291759 & ($23.14 \pm 0.04$, $21.42 \pm 0.01$, $20.60 \pm 0.01$, $20.20 \pm 0.01$, $20.10 \pm 0.04$) & $0.52 \pm 0.03$ \\
DESJ0237-3017 (1) & 39.346808 & -30.292181 & ($21.90 \pm 0.06$, $21.08 \pm 0.04$, $20.23 \pm 0.03$, $19.97 \pm 0.05$, $19.66 \pm 0.11$) & $0.85 \pm 0.07$ \\
\hline
DESJ0238-3334 (A) & 39.554948 & -33.574918 & ($18.06 \pm 0.00$, $17.17 \pm 0.00$, $16.81 \pm 0.00$, $16.57 \pm 0.00$, $16.48 \pm 0.01$) & $0.19 \pm 0.00$ \\
DESJ0238-3334 (1) & 39.554650 & -33.573914 & ($19.98 \pm 0.00$, $19.31 \pm 0.00$, $19.04 \pm 0.00$, $18.87 \pm 0.01$, $18.80 \pm 0.02$) & $0.21 \pm 0.03$ \\
DESJ0238-3334 (2) & 39.554438 & -33.575865 & ($20.82 \pm 0.00$, $20.33 \pm 0.00$, $20.02 \pm 0.01$, $19.96 \pm 0.01$, $19.90 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.20 \pm 0.16$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0239-0127 (A) & 39.926131 & -1.463204 & ($19.30 \pm 0.01$, $18.34 \pm 0.00$, $18.00 \pm 0.00$, $17.67 \pm 0.01$, $17.64 \pm 0.02$) & $0.15 \pm 0.02$ \\
DESJ0239-0127 (1) & 39.926100 & -1.464460 & \ldots & \ldots \\
DESJ0239-0127 (2) & 39.925750 & -1.461500 & \ldots & \ldots \\
\hline
DESJ0239-0134 (A) & 39.971337 & -1.582266 & ($19.72 \pm 0.01$, $17.95 \pm 0.00$, $17.38 \pm 0.00$, $17.08 \pm 0.00$, $16.97 \pm 0.01$) & $0.37 \pm 0.00$ \\
DESJ0239-0134 (1) & 39.973751 & -1.584245 & ($21.45 \pm 0.03$, $20.34 \pm 0.01$, $19.73 \pm 0.01$, $19.62 \pm 0.03$, $19.72 \pm 0.09$) & $0.68 \pm 0.03$ \\
DESJ0239-0134 (2) & 39.970890 & -1.585080 & \ldots & \ldots \\
DESJ0239-0134 (3) & 39.968590 & -1.584570 & \ldots & \ldots \\
\hline
DESJ0242-2132 (A) & 40.649618 & -21.540553 & ($18.34 \pm 0.00$, $16.99 \pm 0.00$, $16.53 \pm 0.00$, $16.21 \pm 0.00$, $16.11 \pm 0.01$) & $0.17 \pm 0.01$ \\
DESJ0242-2132 (1) & 40.655275 & -21.539033 & ($21.44 \pm 0.06$, $20.27 \pm 0.03$, $19.85 \pm 0.03$, $19.99 \pm 0.08$, $19.85 \pm 0.24$) & $0.74 \pm 0.11$ \\
DESJ0242-2132 (2) & 40.651778 & -21.545416 & ($22.74 \pm 0.10$, $21.46 \pm 0.04$, $21.09 \pm 0.05$, $21.00 \pm 0.10$, $21.22 \pm 0.41$) & $0.59 \pm 0.05$ \\
\hline
DESJ0243-3843 (A) & 40.912073 & -48.560811 & ($20.45 \pm 0.01$, $18.64 \pm 0.00$, $17.91 \pm 0.00$, $17.53 \pm 0.00$, $17.39 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.48 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0243-3843 (1) & 40.905940 & -48.562850 & ($21.95 \pm 0.05$, $21.01 \pm 0.03$, $20.35 \pm 0.02$, $20.04 \pm 0.04$, $20.17 \pm 0.13$) & $0.82 \pm 0.07$ \\
DESJ0243-3843 (2) & 40.906390 & -48.559780 & ($22.09 \pm 0.16$, $19.85 \pm 0.03$, $19.22 \pm 0.03$, $18.98 \pm 0.04$, $18.78 \pm 0.11$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.23 \pm 0.11$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0245-5301 (A) & 41.353430 & -53.029290 & ($19.15 \pm 0.01$, $17.69 \pm 0.00$, $17.16 \pm 0.00$, $16.83 \pm 0.00$, $16.70 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.28 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0245-5301 (1) & 41.350660 & -53.030610 & \ldots & \ldots \\
DESJ0245-5301 (2) & 41.352080 & -53.028730 & \ldots & \ldots \\
DESJ0245-5301 (3) & 41.354270 & -53.027290 & \ldots & \ldots \\
\hline
DESJ0248-0331 (A) & 42.014140 & -3.529160 & ($17.19 \pm 0.00$, $15.98 \pm 0.00$, $15.54 \pm 0.00$, $15.23 \pm 0.00$, $15.10 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.19 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0248-0331 (1) & 42.012260 & -3.533050 & \ldots & \ldots \\
DESJ0248-0331 (2) & 42.010300 & -3.531570 & \ldots & \ldots \\
\hline
DESJ0248-0216 (A) & 42.034771 & -2.277023 & ($18.52 \pm 0.00$, $17.20 \pm 0.00$, $16.75 \pm 0.00$, $16.43 \pm 0.00$, $16.32 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.23 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0248-0216 (1) & 42.038470 & -2.278930 & \ldots & \ldots \\
DESJ0248-0216 (2) & 42.038430 & -2.276260 & \ldots & \ldots \\
\hline
DESJ0248-3955 (A) & 42.039764 & -39.930101 & ($21.29 \pm 0.02$, $20.04 \pm 0.01$, $19.06 \pm 0.01$, $18.57 \pm 0.01$, $18.36 \pm 0.02$) & $0.67 \pm 0.02$ \\
DESJ0248-3955 (1) & 42.038798 & -39.930794 & ($22.32 \pm 0.04$, $21.92 \pm 0.04$, $21.42 \pm 0.04$, $21.05 \pm 0.06$, $20.63 \pm 0.14$) & $1.16 \pm 0.15$ \\
DESJ0248-3955 (2) & 42.039712 & -39.931279 & ($22.42 \pm 0.03$, $22.11 \pm 0.03$, $21.43 \pm 0.03$, $21.04 \pm 0.04$, $20.93 \pm 0.12$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.11 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0250-6308 (A) & 42.611700 & -63.145144 & ($23.72 \pm 0.09$, $21.75 \pm 0.02$, $20.71 \pm 0.01$, $20.24 \pm 0.02$, $20.22 \pm 0.06$) & $0.66 \pm 0.05$ \\
DESJ0250-6308 (1) & 42.613363 & -63.144254 & ($21.94 \pm 0.07$, $21.12 \pm 0.04$, $20.38 \pm 0.04$, $20.28 \pm 0.08$, $20.32 \pm 0.25$) & $0.55 \pm 0.24$ \\
\hline
DESJ0251-5515 (A) & 42.954300 & -55.263670 & ($18.45 \pm 0.00$, $17.21 \pm 0.00$, $16.77 \pm 0.00$, $16.46 \pm 0.00$, $16.30 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.22 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0251-5515 (1) & 42.955810 & -55.261960 & \ldots & \ldots \\
\hline
DESJ0252-4732 (A) & 43.082910 & -47.543820 & ($21.28 \pm 0.02$, $19.48 \pm 0.00$, $18.69 \pm 0.00$, $18.12 \pm 0.00$, $17.98 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.49 \pm 0.03$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0252-4732 (1) & 43.081990 & -47.543290 & ($23.02 \pm 0.06$, $21.22 \pm 0.01$, $20.29 \pm 0.01$, $19.43 \pm 0.01$, $19.19 \pm 0.02$) & $0.74 \pm 0.04$ \\
\hline
DESJ0252-1459 (A) & 43.173265 & -14.992111 & ($18.54 \pm 0.00$, $17.22 \pm 0.00$, $16.72 \pm 0.00$, $16.41 \pm 0.00$, $16.31 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.24 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0252-1459 (1) & 43.174150 & -14.992540 & \ldots & \ldots \\
\hline
DESJ0253-2629 (A) & 43.427637 & -26.493435 & ($21.91 \pm 0.02$, $20.13 \pm 0.01$, $19.25 \pm 0.00$, $18.86 \pm 0.01$, $18.74 \pm 0.02$) & $0.56 \pm 0.03$ \\
DESJ0253-2629 (1) & 43.428760 & -26.494251 & ($21.94 \pm 0.06$, $20.91 \pm 0.04$, $20.25 \pm 0.03$, $20.06 \pm 0.06$, $19.90 \pm 0.19$) & $0.47 \pm 0.18$ \\
\hline
DESJ0257-2209 (A) & 44.412121 & -22.157490 & ($21.72 \pm 0.04$, $19.75 \pm 0.01$, $19.18 \pm 0.01$, $18.73 \pm 0.01$, $18.71 \pm 0.04$) & $0.40 \pm 0.06$ \\
DESJ0257-2209 (1) & 44.412520 & -22.157140 & \ldots & \ldots \\
\hline
DESJ0304-4921 (A) & 46.067290 & -49.357250 & ($19.78 \pm 0.01$, $18.03 \pm 0.00$, $17.45 \pm 0.00$, $17.12 \pm 0.00$, $17.01 \pm 0.01$)\textsuperscript{\textdagger} & $0.38 \pm 0.00$\textsuperscript{\textdagger} \\
DESJ0304-4921 (1) & 46.060780 & -49.362830 & ($22.72 \pm 0.08$, $22.11 \pm 0.07$, $21.88 \pm 0.10$, $21.80 \pm 0.16$, $24.32 \pm 5.60$)\textsuperscript{\textdagger} & $0.41 \pm 0.15$\textsuperscript{\textdagger} \\
DESJ0304-4921 (2) & 46.057950 & -49.360240 & ($21.38 \pm 0.04$, $20.51 \pm 0.03$, $20.26 \pm 0.04$, $19.92 \pm 0.06$, $20.11 \pm 0.23$)\textsuperscript{\textdagger} & $0.30 \pm 0.03$\textsuperscript{\textdagger} \\
DESJ0304-4921 (3) & 46.056030 & -49.356300 & ($23.14 \pm 0.08$, $22.39 \pm 0.07$, $22.18 \pm 0.09$, $22.04 \pm 0.14$, $21.91 \pm 0.44$)\textsuperscript{\textdagger} & $0.38 \pm 0.08$\textsuperscript{\textdagger} \\
\hline
DESJ0307-5042 (A) & 46.960540 & -50.701220 & ($21.11 \pm 0.03$, $19.19 \pm 0.01$, $18.31 \pm 0.01$, $17.91 \pm 0.01$, $17.71 \pm 0.03$)\textsuperscript{\textdagger} & $0.61 \pm 0.02$\textsuperscript{\textdagger} \\
DESJ0307-5042 (1) & 46.964710 & -50.698950 & ($22.43 \pm 0.07$, $21.85 \pm 0.05$, $21.67 \pm 0.08$, $21.13 \pm 0.11$, $20.95 \pm 0.32$)\textsuperscript{\textdagger} & $0.99 \pm 0.05$\textsuperscript{\textdagger} \\
DESJ0307-5042 (2) & 46.958910 & -50.698460 & ($21.35 \pm 0.05$, $20.59 \pm 0.03$, $20.01 \pm 0.03$, $19.66 \pm 0.05$, $19.27 \pm 0.14$)\textsuperscript{\textdagger} & $0.69 \pm 0.03$\textsuperscript{\textdagger} \\
\hline
DESJ0309-3805 (A) & 47.335810 & -38.096070 & ($20.99 \pm 0.02$, $19.67 \pm 0.01$, $18.77 \pm 0.01$, $18.29 \pm 0.01$, $18.19 \pm 0.02$) & $0.62 \pm 0.01$ \\
DESJ0309-3805 (1) & 47.335720 & -38.096540 & \ldots & \ldots \\
\hline
DESJ0311-4232 (A) & 47.863261 & -42.538645 & ($19.49 \pm 0.01$, $17.91 \pm 0.00$, $17.38 \pm 0.00$, $17.08 \pm 0.00$, $16.95 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.33 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0311-4232 (1) & 47.862010 & -42.539730 & \ldots & \ldots \\
\hline
DESJ0315-5954 (A) & 48.838290 & -59.913427 & ($20.01 \pm 0.01$, $18.21 \pm 0.00$, $17.62 \pm 0.00$, $17.24 \pm 0.00$, $17.13 \pm 0.01$) & $0.42 \pm 0.01$ \\
DESJ0315-5954 (1) & 48.842350 & -59.914800 & \ldots & \ldots \\
\hline
DESJ0317-4421 (A) & 49.474911 & -44.351994 & ($19.07 \pm 0.00$, $17.68 \pm 0.00$, $17.23 \pm 0.00$, $16.92 \pm 0.00$, $16.80 \pm 0.01$) & $0.24 \pm 0.01$ \\
DESJ0317-4421 (1) & 49.474020 & -44.349920 & ($20.43 \pm 0.02$, $19.50 \pm 0.01$, $19.18 \pm 0.01$, $19.00 \pm 0.02$, $18.86 \pm 0.06$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.15 \pm 0.05$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0327-1326 (A) & 51.863220 & -13.439641 & ($21.64 \pm 0.04$, $19.83 \pm 0.01$, $18.95 \pm 0.01$, $18.49 \pm 0.01$, $18.41 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.58 \pm 0.03$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0327-1326 (B) & 51.863142 & -13.440587 & ($21.85 \pm 0.05$, $20.01 \pm 0.01$, $19.18 \pm 0.01$, $18.77 \pm 0.01$, $18.60 \pm 0.05$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.53 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0327-1326 (C) & 51.864226 & -13.440328 & ($22.76 \pm 0.07$, $21.11 \pm 0.02$, $20.28 \pm 0.02$, $19.89 \pm 0.02$, $19.57 \pm 0.08$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.53 \pm 0.39$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0327-1326 (1) & 51.860735 & -13.437510 & ($20.92 \pm 0.05$, $19.91 \pm 0.03$, $19.41 \pm 0.03$, $19.13 \pm 0.04$, $19.19 \pm 0.23$) & $0.56 \pm 0.20$ \\
DESJ0327-1326 (2) & 51.866482 & -13.435871 & ($20.83 \pm 0.02$, $20.61 \pm 0.02$, $20.39 \pm 0.03$, $20.42 \pm 0.06$, $20.17 \pm 0.23$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $1.49 \pm 0.93$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0327-1326 (3) & 51.863183 & -13.435704 & ($21.20 \pm 0.05$, $20.81 \pm 0.04$, $20.51 \pm 0.06$, $20.17 \pm 0.08$, $99.00 \pm 99.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.97 \pm 0.57$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0327-1326 (4) & 51.867601 & -13.436899 & ($20.96 \pm 0.01$, $20.71 \pm 0.01$, $20.59 \pm 0.03$, $20.45 \pm 0.04$, $19.90 \pm 0.12$) & $1.28 \pm 0.71$ \\
DESJ0327-1326 (5) & 51.868049 & -13.437711 & ($21.40 \pm 0.01$, $21.19 \pm 0.02$, $21.04 \pm 0.03$, $21.00 \pm 0.04$, $20.37 \pm 0.12$) & $0.70 \pm 0.34$ \\
\hline
DESJ0328-2140 (A) & 52.056654 & -21.672092 & ($20.87 \pm 0.03$, $18.96 \pm 0.01$, $18.06 \pm 0.00$, $17.67 \pm 0.01$, $17.51 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.57 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0328-2140 (1) & 52.059798 & -21.668508 & ($20.72 \pm 0.02$, $20.31 \pm 0.02$, $19.94 \pm 0.02$, $19.79 \pm 0.04$, $19.87 \pm 0.14$) & $1.47 \pm 0.82$ \\
DESJ0328-2140 (2) & 52.063308 & -21.674595 & ($22.24 \pm 0.04$, $21.41 \pm 0.02$, $21.10 \pm 0.03$, $21.10 \pm 0.05$, $20.76 \pm 0.13$) & $0.57 \pm 0.04$ \\
DESJ0328-2140 (3) & 52.051870 & -21.667600 & \ldots & \ldots \\
\hline
DESJ0330-5228 (A) & 52.737265 & -52.470270 & ($19.68 \pm 0.01$, $18.13 \pm 0.00$, $17.52 \pm 0.00$, $17.18 \pm 0.01$, $17.07 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.44 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0330-5228 (1) & 52.734562 & -52.470840 & ($21.21 \pm 0.02$, $20.51 \pm 0.02$, $20.08 \pm 0.02$, $19.77 \pm 0.03$, $19.68 \pm 0.09$) & $0.60 \pm 0.18$ \\
DESJ0330-5228 (2) & 52.736680 & -52.471940 & \ldots & \ldots \\
\hline
\hline
DESJ0334-1311 (A) & 53.625435 & -13.186557 & ($19.61 \pm 0.01$, $17.95 \pm 0.00$, $17.40 \pm 0.00$, $17.07 \pm 0.00$, $16.94 \pm 0.01$) & $0.36 \pm 0.01$ \\
DESJ0334-1311 (1) & 53.627340 & -13.185350 & ($21.69 \pm 0.06$, $20.35 \pm 0.03$, $19.88 \pm 0.03$, $19.62 \pm 0.04$, $19.38 \pm 0.15$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.37 \pm 0.18$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0334-1311 (2) & 53.624030 & -13.187360 & \ldots & \ldots \\
\hline
DESJ0336-3812 (A) & 54.119030 & -38.202440 & ($20.10 \pm 0.01$, $18.96 \pm 0.01$, $18.51 \pm 0.01$, $18.16 \pm 0.01$, $17.97 \pm 0.03$) & $0.19 \pm 0.05$ \\
DESJ0336-3812 (1) & 54.119260 & -38.202840 & \ldots & \ldots \\
\hline
DESJ0339-3856 (A) & 54.820713 & -38.950019 & ($21.67 \pm 0.03$, $20.73 \pm 0.02$, $20.03 \pm 0.02$, $19.72 \pm 0.03$, $19.52 \pm 0.07$) & $0.69 \pm 0.05$ \\
DESJ0339-3856 (1) & 54.820060 & -38.949950 & \ldots & \ldots \\
\hline
DESJ0339-3313 (A) & 54.855066 & -33.219260 & ($18.56 \pm 0.00$, $17.10 \pm 0.00$, $16.62 \pm 0.00$, $16.31 \pm 0.00$, $16.17 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.27 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0339-3313 (1) & 54.858179 & -33.221273 & ($20.39 \pm 0.03$, $19.00 \pm 0.01$, $18.63 \pm 0.01$, $18.35 \pm 0.02$, $18.15 \pm 0.06$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.24 \pm 0.20$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0339-4849 (A) & 54.771640 & -48.824750 & ($20.33 \pm 0.02$, $18.52 \pm 0.01$, $17.81 \pm 0.01$, $17.42 \pm 0.01$, $17.28 \pm 0.02$)\textsuperscript{\textdagger} & $0.47 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0339-4849 (1) & 54.771290 & -48.821540 & ($21.83 \pm 0.07$, $20.75 \pm 0.03$, $20.20 \pm 0.04$, $19.81 \pm 0.06$, $19.43 \pm 0.11$)\textsuperscript{\textdagger} & $0.76 \pm 0.05$\textsuperscript{\textdagger} \\
DESJ0339-4849 (2) & 54.777430 & -48.824710 & ($22.52 \pm 0.06$, $22.26 \pm 0.06$, $22.47 \pm 0.14$, $22.31 \pm 0.23$, $23.49 \pm 2.11$)\textsuperscript{\textdagger} & $0.57 \pm 0.20$\textsuperscript{\textdagger} \\
\hline
DESJ0341-5130 (A) & 55.378330 & -51.512410 & ($20.85 \pm 0.02$, $19.53 \pm 0.01$, $19.01 \pm 0.01$, $18.66 \pm 0.01$, $18.56 \pm 0.03$)\textsuperscript{\textdagger} & $0.32 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0341-5130 (1) & 55.378490 & -51.513120 & \ldots & \ldots \\
\hline
DESJ0342-5355A (A) & 55.519200 & -53.920590 & ($21.12 \pm 0.03$, $19.17 \pm 0.01$, $18.37 \pm 0.01$, $17.94 \pm 0.01$, $17.88 \pm 0.02$)\textsuperscript{\textdagger} & $0.52 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0342-5355A (1) & 55.517110 & -53.920430 & ($24.61 \pm 0.20$, $22.43 \pm 0.04$, $21.47 \pm 0.02$, $20.84 \pm 0.03$, $20.69 \pm 0.08$)\textsuperscript{\textdagger} & $0.67 \pm 0.05$\textsuperscript{\textdagger} \\
\hline
DESJ0342-5355B (A) & 55.519200 & -53.920590 & ($21.12 \pm 0.03$, $19.17 \pm 0.01$, $18.37 \pm 0.01$, $17.94 \pm 0.01$, $17.88 \pm 0.02$)\textsuperscript{\textdagger} & $0.52 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0342-5355B (1) & 55.524060 & -53.921550 & ($22.43 \pm 0.07$, $21.88 \pm 0.06$, $21.50 \pm 0.06$, $21.34 \pm 0.12$, $99.00 \pm 99.00$)\textsuperscript{\textdagger} & $0.22 \pm 0.08$\textsuperscript{\textdagger} \\
DESJ0342-5355B (2) & 55.523270 & -53.922750 & ($23.35 \pm 0.11$, $22.92 \pm 0.10$, $22.79 \pm 0.13$, $23.26 \pm 0.46$, $99.00 \pm 99.00$)\textsuperscript{\textdagger} & $0.94 \pm 0.24$\textsuperscript{\textdagger} \\
\hline
DESJ0342-2342 (A) & 55.700910 & -23.712895 & ($22.95 \pm 0.08$, $21.01 \pm 0.02$, $19.82 \pm 0.01$, $19.32 \pm 0.01$, $19.15 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.75 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0342-2342 (1) & 55.701260 & -23.714200 & ($23.36 \pm 0.14$, $22.31 \pm 0.07$, $21.48 \pm 0.06$, $21.07 \pm 0.08$, $21.16 \pm 0.29$) & $0.67 \pm 0.08$ \\
DESJ0342-2342 (2) & 55.702741 & -23.712527 & ($23.39 \pm 0.09$, $22.93 \pm 0.07$, $22.09 \pm 0.07$, $21.93 \pm 0.11$, $21.89 \pm 0.33$) & $0.86 \pm 0.08$ \\
\hline
DESJ0345-3403 (A) & 56.262870 & -34.050482 & ($17.96 \pm 0.00$, $16.64 \pm 0.00$, $16.20 \pm 0.00$, $15.90 \pm 0.00$, $15.77 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.24 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0345-3403 (1) & 56.258904 & -34.048696 & ($20.77 \pm 0.02$, $19.90 \pm 0.01$, $19.66 \pm 0.02$, $19.49 \pm 0.03$, $19.37 \pm 0.08$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.21 \pm 0.08$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0345-3403 (2) & 56.263530 & -34.052110 & \ldots & \ldots \\
\hline
DESJ0348-2145 (A) & 57.009697 & -21.750830 & ($19.37 \pm 0.01$, $17.74 \pm 0.00$, $17.14 \pm 0.00$, $16.82 \pm 0.00$, $16.67 \pm 0.01$) & $0.35 \pm 0.01$ \\
DESJ0348-2145 (1) & 57.011305 & -21.748653 & ($21.81 \pm 0.05$, $20.74 \pm 0.02$, $20.29 \pm 0.03$, $19.95 \pm 0.04$, $19.77 \pm 0.11$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.57 \pm 0.18$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0348-2145 (2) & 57.007940 & -21.749350 & \ldots & \ldots \\
\hline
\hline
DESJ0352-3825 (A) & 58.176701 & -38.429152 & ($20.49 \pm 0.02$, $19.12 \pm 0.01$, $18.44 \pm 0.01$, $18.07 \pm 0.01$, $17.99 \pm 0.02$)\textsuperscript{\textdagger} & $0.51 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0352-3825 (1) & 58.177612 & -38.429411 & ($21.71 \pm 0.02$, $21.04 \pm 0.01$, $20.78 \pm 0.02$, $20.55 \pm 0.03$, $20.65 \pm 0.10$)\textsuperscript{\textdagger} & $0.28 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0352-3825 (2) & 58.175870 & -38.429900 & \ldots & \ldots \\
DESJ0352-3825 (3) & 58.176480 & -38.428270 & \ldots & \ldots \\
\hline
DESJ0354-4446 (A) & 58.559041 & -44.768957 & ($20.09 \pm 0.01$, $18.46 \pm 0.00$, $17.90 \pm 0.00$, $17.57 \pm 0.00$, $17.44 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.34 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0354-4446 (1) & 58.557800 & -44.768370 & \ldots & \ldots \\
\hline
DESJ0356-5607 (A) & 59.026020 & -56.124830 & ($19.89 \pm 0.01$, $18.18 \pm 0.00$, $17.56 \pm 0.00$, $17.19 \pm 0.00$, $17.09 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.42 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0356-5607 (1) & 59.025930 & -56.125820 & \ldots & \ldots \\
DESJ0356-5607 (2) & 59.027570 & -56.124020 & \ldots & \ldots \\
\hline
DESJ0356-2408 (A) & 59.204420 & -24.144760 & ($20.45 \pm 0.02$, $19.18 \pm 0.01$, $18.62 \pm 0.01$, $18.27 \pm 0.01$, $18.15 \pm 0.03$) & $0.39 \pm 0.04$ \\
DESJ0356-2408 (B) & 59.204270 & -24.142970 & ($21.16 \pm 0.02$, $19.94 \pm 0.01$, $19.38 \pm 0.01$, $19.08 \pm 0.01$, $18.98 \pm 0.05$) & $0.52 \pm 0.05$ \\
DESJ0356-2408 (1) & 59.203970 & -24.145250 & \ldots & \ldots \\
DESJ0356-2408 (2) & 59.203660 & -24.143710 & \ldots & \ldots \\
DESJ0356-2408 (3) & 59.203670 & -24.142620 & \ldots & \ldots \\
\hline
DESJ0357-4756 (A) & 59.307560 & -47.946310 & ($19.01 \pm 0.00$, $17.53 \pm 0.00$, $17.04 \pm 0.00$, $16.73 \pm 0.00$, $16.59 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.27 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0357-4756 (B) & 59.306550 & -47.948000 & ($18.48 \pm 0.00$, $17.12 \pm 0.00$, $16.63 \pm 0.00$, $16.33 \pm 0.00$, $16.18 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.26 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0357-4756 (1) & 59.305090 & -47.948510 & \ldots & \ldots \\
DESJ0357-4756 (2) & 59.308520 & -47.944370 & \ldots & \ldots \\
\hline
DESJ0358-2415 (A) & 59.694269 & -24.254620 & ($21.76 \pm 0.04$, $19.76 \pm 0.01$, $18.76 \pm 0.01$, $18.30 \pm 0.01$, $18.14 \pm 0.02$) & $0.61 \pm 0.02$ \\
DESJ0358-2415 (1) & 59.696760 & -24.252230 & \ldots & \ldots \\
DESJ0358-2415 (2) & 59.694100 & -24.250670 & \ldots & \ldots \\
\hline
DESJ0359-2433 (A) & 59.985108 & -24.565205 & ($18.08 \pm 0.00$, $16.75 \pm 0.00$, $16.29 \pm 0.00$, $15.98 \pm 0.00$, $15.83 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.22 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0359-2433 (1) & 59.988067 & -24.564242 & ($20.28 \pm 0.01$, $19.22 \pm 0.00$, $18.77 \pm 0.00$, $18.44 \pm 0.01$, $18.24 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.08 \pm 0.03$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0402-2205 (A) & 60.523829 & -22.098986 & ($21.75 \pm 0.02$, $20.00 \pm 0.00$, $19.31 \pm 0.00$, $18.94 \pm 0.01$, $18.82 \pm 0.02$) & $0.47 \pm 0.05$ \\
DESJ0402-2205 (B) & 60.523358 & -22.099456 & ($21.95 \pm 0.02$, $20.31 \pm 0.00$, $19.66 \pm 0.00$, $19.30 \pm 0.01$, $19.19 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.45 \pm 0.18$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0402-2205 (1) & 60.522730 & -22.099970 & \ldots & \ldots \\
\hline
DESJ0403-5057 (A) & 60.786770 & -50.965686 & ($22.37 \pm 0.04$, $20.64 \pm 0.01$, $19.82 \pm 0.01$, $19.44 \pm 0.01$, $19.27 \pm 0.04$) & $0.56 \pm 0.03$ \\
DESJ0403-5057 (1) & 60.786002 & -50.966614 & ($23.30 \pm 0.09$, $21.96 \pm 0.03$, $21.45 \pm 0.04$, $21.29 \pm 0.06$, $21.06 \pm 0.18$) & $0.45 \pm 0.12$ \\
DESJ0403-5057 (2) & 60.788293 & -50.966506 & ($23.66 \pm 0.13$, $22.63 \pm 0.06$, $22.02 \pm 0.06$, $21.99 \pm 0.12$, $22.05 \pm 0.46$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.56 \pm 0.23$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0406-2254 (A) & 61.553430 & -22.903376 & ($22.57 \pm 0.06$, $20.81 \pm 0.01$, $19.63 \pm 0.01$, $19.02 \pm 0.01$, $18.89 \pm 0.03$) & $0.81 \pm 0.02$ \\
DESJ0406-2254 (1) & 61.552137 & -22.903098 & ($23.28 \pm 0.14$, $21.96 \pm 0.05$, $21.39 \pm 0.05$, $21.26 \pm 0.09$, $20.70 \pm 0.19$) & $0.51 \pm 0.07$ \\
DESJ0406-2254 (2) & 61.553311 & -22.904896 & ($23.62 \pm 0.12$, $22.48 \pm 0.05$, $22.07 \pm 0.07$, $22.07 \pm 0.12$, $21.76 \pm 0.33$) & $0.51 \pm 0.07$ \\
\hline
DESJ0411-4506 (A) & 62.792039 & -45.107710 & ($19.41 \pm 0.01$, $18.19 \pm 0.00$, $17.75 \pm 0.00$, $17.45 \pm 0.00$, $17.33 \pm 0.01$) & $0.21 \pm 0.01$ \\
DESJ0411-4506 (1) & 62.791850 & -45.108873 & ($20.91 \pm 0.01$, $20.00 \pm 0.01$, $19.59 \pm 0.01$, $19.39 \pm 0.01$, $19.12 \pm 0.04$) & $0.24 \pm 0.04$ \\
\hline
DESJ0411-4819 (A) & 62.795720 & -48.327663 & ($19.93 \pm 0.01$, $18.35 \pm 0.00$, $17.74 \pm 0.00$, $17.39 \pm 0.00$, $17.28 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.36 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0411-4819 (1) & 62.793929 & -48.329058 & ($21.74 \pm 0.02$, $20.76 \pm 0.01$, $20.21 \pm 0.01$, $19.92 \pm 0.02$, $19.81 \pm 0.05$) & $0.65 \pm 0.06$ \\
DESJ0411-4819 (2) & 62.792607 & -48.327323 & ($22.21 \pm 0.05$, $21.06 \pm 0.02$, $20.61 \pm 0.03$, $20.28 \pm 0.04$, $20.00 \pm 0.10$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.73 \pm 0.17$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0413-1958 (A) & 63.295501 & -19.884891 & ($22.75 \pm 0.06$, $20.93 \pm 0.02$, $19.87 \pm 0.01$, $19.39 \pm 0.01$, $19.05 \pm 0.03$) & $0.67 \pm 0.03$ \\
DESJ0413-1958 (1) & 63.294756 & -19.884400 & ($23.15 \pm 0.07$, $22.08 \pm 0.04$, $21.39 \pm 0.04$, $21.20 \pm 0.05$, $20.85 \pm 0.15$) & $0.64 \pm 0.10$ \\
DESJ0413-1958 (2) & 63.295377 & -19.883911 & ($23.66 \pm 0.11$, $22.51 \pm 0.05$, $21.87 \pm 0.05$, $21.76 \pm 0.09$, $20.84 \pm 0.14$) & $0.57 \pm 0.10$ \\
DESJ0413-1958 (3) & 63.294535 & -19.885060 & ($23.76 \pm 0.13$, $22.82 \pm 0.07$, $22.23 \pm 0.08$, $21.67 \pm 0.08$, $21.89 \pm 0.39$) & $0.61 \pm 0.13$ \\
\hline
DESJ0413-5117 (A) & 63.348725 & -51.297361 & ($21.08 \pm 0.02$, $20.57 \pm 0.02$, $20.20 \pm 0.02$, $19.45 \pm 0.02$, $18.86 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.96 \pm 0.13$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0413-5117 (1) & 63.349806 & -51.296982 & ($21.04 \pm 0.02$, $20.59 \pm 0.02$, $20.43 \pm 0.02$, $19.75 \pm 0.03$, $18.77 \pm 0.04$) & $0.56 \pm 0.17$ \\
\hline
DESJ0415-4143 (A) & 63.935540 & -41.729490 & ($22.35 \pm 0.08$, $20.46 \pm 0.03$, $19.22 \pm 0.02$, $18.70 \pm 0.02$, $18.46 \pm 0.04$)\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} & $0.72 \pm 0.01$\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} \\
DESJ0415-4143 (1) & 63.933290 & -41.730270 & ($21.36 \pm 0.05$, $21.03 \pm 0.06$, $20.45 \pm 0.07$, $19.93 \pm 0.07$, $19.64 \pm 0.16$)\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} & $0.94 \pm 0.05$\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} \\
DESJ0415-4143 (2) & 63.933020 & -41.729400 & \ldots & \ldots \\
\hline
DESJ0416-2404 (A) & 64.032053 & -24.077430 & ($19.77 \pm 0.01$, $17.94 \pm 0.00$, $17.38 \pm 0.00$, $17.04 \pm 0.00$, $16.95 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.40 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0416-2404 (1) & 64.032870 & -24.076070 & \ldots & \ldots \\
\hline
DESJ0416-5525 (A) & 64.186786 & -55.416745 & ($19.71 \pm 0.01$, $18.08 \pm 0.00$, $17.49 \pm 0.00$, $17.18 \pm 0.01$, $16.99 \pm 0.02$) & $0.37 \pm 0.01$ \\
DESJ0416-5525 (1) & 64.186830 & -55.417950 & \ldots & \ldots \\
\hline
DESJ0422-2803 (A) & 65.644655 & -28.065193 & ($21.78 \pm 0.04$, $20.06 \pm 0.01$, $19.06 \pm 0.01$, $18.52 \pm 0.01$, $18.26 \pm 0.03$) & $0.61 \pm 0.02$ \\
DESJ0422-2803 (1) & 65.643960 & -28.064850 & \ldots & \ldots \\
\hline
DESJ0424-3317 (A) & 66.161210 & -33.294908 & ($20.21 \pm 0.01$, $18.96 \pm 0.00$, $18.17 \pm 0.00$, $17.75 \pm 0.00$, $17.65 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.52 \pm 0.08$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0424-3317 (1) & 66.160103 & -33.293741 & ($21.20 \pm 0.04$, $20.16 \pm 0.02$, $19.56 \pm 0.02$, $19.21 \pm 0.03$, $19.20 \pm 0.09$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.69 \pm 0.18$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0424-3317 (2) & 66.162250 & -33.296202 & ($20.94 \pm 0.03$, $20.27 \pm 0.02$, $19.71 \pm 0.02$, $19.30 \pm 0.02$, $19.17 \pm 0.07$) & $0.54 \pm 0.18$ \\
\hline
DESJ0438-3220 (A) & 69.564118 & -32.347451 & ($20.97 \pm 0.02$, $19.25 \pm 0.01$, $18.57 \pm 0.01$, $18.20 \pm 0.01$, $18.16 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.49 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0438-3220 (1) & 69.565086 & -32.346385 & ($22.70 \pm 0.05$, $21.82 \pm 0.03$, $21.13 \pm 0.03$, $20.82 \pm 0.04$, $20.62 \pm 0.13$) & $0.73 \pm 0.06$ \\
\hline
DESJ0440-2658 (A) & 70.192775 & -26.975391 & ($20.57 \pm 0.02$, $18.83 \pm 0.01$, $18.10 \pm 0.01$, $17.71 \pm 0.01$, $17.56 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.50 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0440-2658 (1) & 70.193860 & -26.973023 & ($23.10 \pm 0.12$, $21.77 \pm 0.05$, $21.41 \pm 0.07$, $21.06 \pm 0.09$, $20.60 \pm 0.16$) & $0.61 \pm 0.19$ \\
DESJ0440-2658 (2) & 70.196370 & -26.976190 & \ldots & \ldots \\
\hline
DESJ0440-4657 (A) & 70.228709 & -46.959538 & ($20.13 \pm 0.01$, $18.57 \pm 0.00$, $18.06 \pm 0.00$, $17.72 \pm 0.01$, $17.61 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.32 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0440-4657 (B) & 70.226852 & -46.959930 & ($20.51 \pm 0.01$, $18.94 \pm 0.00$, $18.43 \pm 0.00$, $18.11 \pm 0.01$, $17.99 \pm 0.02$) & $0.32 \pm 0.02$ \\
DESJ0440-4657 (1) & 70.227117 & -46.961590 & ($21.08 \pm 0.03$, $20.03 \pm 0.02$, $19.66 \pm 0.02$, $19.39 \pm 0.03$, $19.04 \pm 0.07$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.38 \pm 0.10$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
\hline
DESJ0448-3019 (A) & 72.052837 & -30.330843 & ($22.83 \pm 0.10$, $20.56 \pm 0.02$, $19.27 \pm 0.01$, $18.79 \pm 0.01$, $18.68 \pm 0.03$) & $0.76 \pm 0.02$ \\
DESJ0448-3019 (1) & 72.056279 & -30.333184 & ($22.00 \pm 0.03$, $21.94 \pm 0.04$, $21.90 \pm 0.08$, $21.77 \pm 0.13$, $21.99 \pm 0.51$) & $0.85 \pm 0.65$ \\
DESJ0448-3019 (2) & 72.057144 & -30.331926 & ($22.68 \pm 0.05$, $22.38 \pm 0.05$, $22.09 \pm 0.08$, $21.86 \pm 0.11$, $21.65 \pm 0.31$) & $0.59 \pm 0.42$ \\
DESJ0448-3019 (3) & 72.055567 & -30.334070 & ($22.58 \pm 0.04$, $22.34 \pm 0.04$, $22.14 \pm 0.07$, $22.22 \pm 0.12$, $22.24 \pm 0.41$) & $0.72 \pm 0.44$ \\
\hline
DESJ0451-1856 (A) & 72.998665 & -18.943611 & ($19.42 \pm 0.01$, $17.75 \pm 0.00$, $17.16 \pm 0.00$, $16.81 \pm 0.00$, $16.67 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.34 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0451-1856 (1) & 72.999780 & -18.949600 & \ldots & \ldots \\
\hline
DESJ0453-4120 (A) & 73.293994 & -41.347261 & ($20.20 \pm 0.01$, $19.31 \pm 0.01$, $18.76 \pm 0.01$, $18.51 \pm 0.01$, $18.34 \pm 0.03$) & $0.22 \pm 0.03$ \\
DESJ0453-4120 (1) & 73.293270 & -41.347550 & \ldots & \ldots \\
\hline
DESJ0453-3639 (A) & 73.498110 & -36.660652 & ($21.32 \pm 0.02$, $20.01 \pm 0.01$, $19.51 \pm 0.01$, $19.21 \pm 0.01$, $19.09 \pm 0.04$) & $0.43 \pm 0.06$ \\
DESJ0453-3639 (1) & 73.497096 & -36.661048 & ($21.11 \pm 0.01$, $20.51 \pm 0.01$, $20.22 \pm 0.01$, $20.12 \pm 0.03$, $20.36 \pm 0.15$) & $0.23 \pm 0.04$ \\
\hline
DESJ0455-2530 (A) & 73.903051 & -25.512790 & ($19.87 \pm 0.01$, $18.17 \pm 0.00$, $17.61 \pm 0.00$, $17.25 \pm 0.01$, $17.22 \pm 0.02$) & $0.33 \pm 0.02$ \\
DESJ0455-2530 (1) & 73.907760 & -25.512129 & ($22.37 \pm 0.07$, $21.30 \pm 0.03$, $21.17 \pm 0.06$, $21.02 \pm 0.09$, $22.29 \pm 1.05$) & $0.42 \pm 0.11$ \\
DESJ0455-2530 (2) & 73.907731 & -25.514455 & ($22.60 \pm 0.08$, $21.59 \pm 0.04$, $21.33 \pm 0.06$, $20.98 \pm 0.08$, $22.50 \pm 1.23$) & $0.49 \pm 0.21$ \\
DESJ0455-2530 (3) & 73.904931 & -25.508571 & ($23.37 \pm 0.22$, $21.65 \pm 0.06$, $21.47 \pm 0.10$, $21.32 \pm 0.16$, $21.84 \pm 0.96$) & $0.42 \pm 0.08$ \\
\hline
DESJ0459-3756 (A) & 74.928720 & -37.936283 & ($20.31 \pm 0.01$, $18.57 \pm 0.00$, $17.87 \pm 0.00$, $17.47 \pm 0.00$, $17.32 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.48 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0459-3756 (1) & 74.925894 & -37.937523 & ($21.89 \pm 0.11$, $20.26 \pm 0.03$, $19.82 \pm 0.04$, $19.48 \pm 0.05$, $19.50 \pm 0.19$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.37 \pm 0.07$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0501-2425 (A) & 75.283044 & -24.420772 & ($20.14 \pm 0.01$, $18.58 \pm 0.00$, $18.06 \pm 0.00$, $17.72 \pm 0.00$, $17.61 \pm 0.01$) & $0.31 \pm 0.02$ \\
DESJ0501-2425 (1) & 75.275220 & -24.418100 & \ldots & \ldots \\
\hline
\hline
DESJ0509-5342 (A) & 77.339140 & -53.703510 & ($20.71 \pm 0.03$, $18.95 \pm 0.01$, $18.32 \pm 0.01$, $17.96 \pm 0.01$, $17.85 \pm 0.03$)\textsuperscript{\textdagger} & $0.42 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ0509-5342 (1) & 77.335550 & -53.702370 & ($21.83 \pm 0.04$, $21.34 \pm 0.04$, $21.20 \pm 0.06$, $21.06 \pm 0.10$, $21.91 \pm 0.74$)\textsuperscript{\textdagger} & $0.26 \pm 0.11$\textsuperscript{\textdagger} \\
DESJ0509-5342 (2) & 77.335430 & -53.705370 & ($22.72 \pm 0.08$, $22.14 \pm 0.06$, $21.95 \pm 0.09$, $22.11 \pm 0.22$, $23.61 \pm 2.91$)\textsuperscript{\textdagger} & $0.14 \pm 0.08$\textsuperscript{\textdagger} \\
\hline
DESJ0510-3232 (A) & 77.553280 & -32.534930 & ($20.44 \pm 0.02$, $19.00 \pm 0.01$, $18.34 \pm 0.01$, $17.97 \pm 0.01$, $17.90 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.32 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0510-3232 (1) & 77.552410 & -32.534210 & \ldots & \ldots \\
DESJ0510-3232 (2) & 77.553520 & -32.536050 & \ldots & \ldots \\
\hline
DESJ0512-3847 (A) & 78.242623 & -38.792068 & ($19.37 \pm 0.00$, $17.79 \pm 0.00$, $17.24 \pm 0.00$, $16.91 \pm 0.00$, $16.75 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.31 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0512-3847 (1) & 78.246990 & -38.785190 & \ldots & \ldots \\
DESJ0512-3847 (2) & 78.234510 & -38.790660 & \ldots & \ldots \\
DESJ0512-3847 (3) & 78.232450 & -38.789700 & \ldots & \ldots \\
DESJ0512-3847 (4) & 78.252310 & -38.797980 & \ldots & \ldots \\
\hline
DESJ0513-2128 (A) & 78.355776 & -21.474701 & ($20.05 \pm 0.04$, $18.59 \pm 0.01$, $18.05 \pm 0.01$, $17.79 \pm 0.02$, $17.89 \pm 0.08$) & $0.35 \pm 0.04$ \\
DESJ0513-2128 (1) & 78.354730 & -21.475840 & \ldots & \ldots \\
\hline
DESJ0513-3050 (A) & 78.356147 & -30.843306 & ($19.70 \pm 0.01$, $18.25 \pm 0.00$, $17.71 \pm 0.00$, $17.39 \pm 0.01$, $17.20 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.34 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0513-3050 (1) & 78.354330 & -30.843450 & \ldots & \ldots \\
DESJ0513-3050 (2) & 78.356250 & -30.841480 & \ldots & \ldots \\
\hline
DESJ0514-5142 (A) & 78.511936 & -51.706105 & ($21.78 \pm 0.04$, $20.14 \pm 0.01$, $19.39 \pm 0.01$, $18.95 \pm 0.01$, $18.78 \pm 0.05$) & $0.54 \pm 0.03$ \\
DESJ0514-5142 (1) & 78.509679 & -51.705679 & ($21.06 \pm 0.02$, $19.98 \pm 0.01$, $19.64 \pm 0.01$, $19.45 \pm 0.02$, $19.13 \pm 0.06$) & $0.27 \pm 0.08$ \\
\hline
DESJ0516-2208 (A) & 79.013227 & -22.146417 & ($21.17 \pm 0.04$, $19.51 \pm 0.01$, $18.67 \pm 0.01$, $18.26 \pm 0.01$, $18.06 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.62 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0516-2208 (1) & 79.013910 & -22.146220 & \ldots & \ldots \\
\hline
DESJ0517-2526 (A) & 79.322430 & -25.444955 & ($20.74 \pm 0.02$, $19.16 \pm 0.01$, $18.53 \pm 0.01$, $18.22 \pm 0.01$, $18.13 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.41 \pm 0.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0517-2526 (1) & 79.322823 & -25.446518 & ($21.38 \pm 0.02$, $20.65 \pm 0.02$, $20.31 \pm 0.02$, $20.25 \pm 0.04$, $20.19 \pm 0.13$) & $0.22 \pm 0.05$ \\
\hline
DESJ0518-4348 (A) & 79.647974 & -43.813522 & ($19.52 \pm 0.00$, $18.71 \pm 0.00$, $18.33 \pm 0.00$, $18.10 \pm 0.00$, $18.02 \pm 0.01$) & $0.15 \pm 0.03$ \\
DESJ0518-4348 (1) & 79.648015 & -43.812478 & ($19.41 \pm 0.00$, $18.77 \pm 0.00$, $18.48 \pm 0.00$, $18.34 \pm 0.01$, $18.30 \pm 0.03$) & $0.14 \pm 0.03$ \\
\hline
DESJ0524-2721 (A) & 81.098610 & -27.353150 & ($19.10 \pm 0.01$, $17.59 \pm 0.00$, $17.06 \pm 0.00$, $16.75 \pm 0.00$, $16.65 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.32 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0524-2721 (1) & 81.099620 & -27.354860 & \ldots & \ldots \\
DESJ0524-2721 (2) & 81.100460 & -27.353640 & \ldots & \ldots \\
\hline
DESJ0525-3712 (A) & 81.477518 & -37.204176 & ($20.30 \pm 0.02$, $18.53 \pm 0.00$, $17.88 \pm 0.00$, $17.52 \pm 0.01$, $17.39 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.44 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0525-3712 (1) & 81.476570 & -37.202830 & \ldots & \ldots \\
\hline
DESJ0527-1858 (A) & 81.754736 & -18.967375 & ($20.66 \pm 0.02$, $18.78 \pm 0.00$, $18.12 \pm 0.00$, $17.76 \pm 0.00$, $17.63 \pm 0.02$) & $0.43 \pm 0.02$ \\
DESJ0527-1858 (1) & 81.756341 & -18.966930 & ($24.25 \pm 0.92$, $20.70 \pm 0.04$, $20.23 \pm 0.05$, $19.89 \pm 0.06$, $19.52 \pm 0.18$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.38 \pm 0.18$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0527-1858 (2) & 81.754372 & -18.965780 & ($22.17 \pm 0.04$, $21.35 \pm 0.02$, $20.91 \pm 0.03$, $20.72 \pm 0.04$, $20.60 \pm 0.15$) & $0.52 \pm 0.27$ \\
DESJ0527-1858 (3) & 81.752815 & -18.969013 & ($22.65 \pm 0.14$, $21.35 \pm 0.05$, $20.95 \pm 0.06$, $20.85 \pm 0.10$, $21.44 \pm 0.75$) & $0.65 \pm 0.61$ \\
\hline
DESJ0528-2633 (A) & 82.154815 & -26.566660 & ($23.26 \pm 0.09$, $21.71 \pm 0.02$, $20.66 \pm 0.02$, $20.01 \pm 0.02$, $19.85 \pm 0.05$) & $0.89 \pm 0.02$ \\
DESJ0528-2633 (1) & 82.153518 & -26.567671 & ($22.20 \pm 0.04$, $21.59 \pm 0.03$, $21.37 \pm 0.04$, $21.15 \pm 0.07$, $20.86 \pm 0.15$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.36 \pm 0.19$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0528-2633 (2) & 82.155330 & -26.567620 & \ldots & \ldots \\
\hline
DESJ0528-3958 (A) & 82.165707 & -39.977586 & ($20.94 \pm 0.02$, $19.18 \pm 0.00$, $18.53 \pm 0.00$, $18.14 \pm 0.01$, $18.02 \pm 0.02$) & $0.44 \pm 0.02$ \\
DESJ0528-3958 (1) & 82.167226 & -39.977522 & ($23.10 \pm 0.06$, $21.96 \pm 0.03$, $21.42 \pm 0.03$, $21.08 \pm 0.05$, $20.99 \pm 0.15$) & $0.59 \pm 0.14$ \\
DESJ0528-3958 (2) & 82.166511 & -39.978731 & ($22.98 \pm 0.07$, $22.03 \pm 0.05$, $21.46 \pm 0.05$, $21.11 \pm 0.07$, $20.62 \pm 0.15$) & $0.82 \pm 0.11$ \\
DESJ0528-3958 (3) & 82.164626 & -39.979112 & ($23.37 \pm 0.16$, $22.49 \pm 0.11$, $21.65 \pm 0.08$, $21.33 \pm 0.12$, $20.55 \pm 0.21$) & $0.60 \pm 0.14$ \\
DESJ0528-3958 (4) & 82.164082 & -39.976435 & ($23.13 \pm 0.13$, $22.07 \pm 0.07$, $21.64 \pm 0.08$, $21.06 \pm 0.10$, $21.39 \pm 0.48$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.63 \pm 0.15$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0531-3158 (A) & 82.926940 & -31.980920 & ($21.15 \pm 0.04$, $19.41 \pm 0.01$, $18.68 \pm 0.01$, $18.29 \pm 0.02$, $18.22 \pm 0.12$)\textsuperscript{\textdagger} & $0.51 \pm 0.02$\textsuperscript{\textdagger} \\
DESJ0531-3158 (1) & 82.925720 & -31.979860 & ($21.92 \pm 0.07$, $20.95 \pm 0.04$, $20.44 \pm 0.05$, $20.14 \pm 0.08$, $19.92 \pm 0.47$)\textsuperscript{\textdagger} & $0.70 \pm 0.04$\textsuperscript{\textdagger} \\
\hline
\hline
DESJ0540-2127 (A) & 85.207056 & -21.459826 & ($21.37 \pm 0.03$, $19.40 \pm 0.01$, $18.60 \pm 0.01$, $18.20 \pm 0.01$, $18.13 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.53 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0540-2127 (1) & 85.210093 & -21.456899 & ($21.00 \pm 0.02$, $20.57 \pm 0.01$, $20.41 \pm 0.02$, $20.50 \pm 0.04$, $20.78 \pm 0.20$) & $0.94 \pm 0.58$ \\
DESJ0540-2127 (2) & 85.210731 & -21.457921 & ($22.05 \pm 0.03$, $21.30 \pm 0.02$, $20.97 \pm 0.02$, $20.98 \pm 0.05$, $21.34 \pm 0.23$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.33 \pm 0.16$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0545-2635 (A) & 86.306553 & -26.588390 & ($19.08 \pm 0.00$, $17.54 \pm 0.00$, $17.03 \pm 0.00$, $16.71 \pm 0.00$, $16.55 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.29 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0545-2635 (B) & 86.306267 & -26.588956 & ($19.86 \pm 0.01$, $18.31 \pm 0.00$, $17.81 \pm 0.00$, $17.47 \pm 0.00$, $17.33 \pm 0.01$) & $0.27 \pm 0.03$ \\
DESJ0545-2635 (1) & 86.305968 & -26.584750 & ($19.45 \pm 0.02$, $18.16 \pm 0.01$, $17.77 \pm 0.01$, $17.60 \pm 0.02$, $17.72 \pm 0.07$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.11 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0545-2635 (2) & 86.309100 & -26.585410 & \ldots & \ldots \\
\hline
DESJ0548-3614 (A) & 87.152364 & -36.242695 & ($18.75 \pm 0.00$, $17.28 \pm 0.00$, $16.76 \pm 0.00$, $16.45 \pm 0.00$, $16.31 \pm 0.01$) & $0.29 \pm 0.01$ \\
DESJ0548-3614 (1) & 87.154760 & -36.243080 & \ldots & \ldots \\
\hline
DESJ0553-3342 (A) & 88.330328 & -33.707007 & ($19.55 \pm 0.01$, $17.72 \pm 0.00$, $16.61 \pm 0.00$, $16.01 \pm 0.00$, $15.83 \pm 0.00$) & $0.37 \pm 0.05$ \\
DESJ0553-3342 (1) & 88.327334 & -33.710146 & ($99.00 \pm 99.00$, $21.98 \pm 0.08$, $20.69 \pm 0.04$, $19.70 \pm 0.03$, $19.49 \pm 0.09$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $1.01 \pm 0.05$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0553-3342 (2) & 88.327140 & -33.707100 & \ldots & \ldots \\
DESJ0553-3342 (3) & 88.327280 & -33.705710 & \ldots & \ldots \\
\hline
DESJ0603-3558 (A) & 90.985450 & -35.968253 & ($20.76 \pm 0.01$, $18.95 \pm 0.00$, $18.21 \pm 0.00$, $17.82 \pm 0.00$, $17.70 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.49 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0603-3558 (1) & 90.981916 & -35.964634 & ($21.70 \pm 0.04$, $20.63 \pm 0.02$, $19.98 \pm 0.02$, $19.48 \pm 0.02$, $19.66 \pm 0.09$) & $0.79 \pm 0.04$ \\
DESJ0603-3558 (2) & 90.980725 & -35.969991 & ($21.10 \pm 0.03$, $20.63 \pm 0.03$, $20.30 \pm 0.03$, $19.99 \pm 0.05$, $20.45 \pm 0.26$) & $0.86 \pm 0.19$ \\
DESJ0603-3558 (3) & 90.991096 & -35.966745 & ($22.12 \pm 0.04$, $21.85 \pm 0.04$, $21.56 \pm 0.05$, $21.18 \pm 0.07$, $20.80 \pm 0.17$) & $1.22 \pm 0.14$ \\
\hline
DESJ0604-3347 (A) & 91.060374 & -33.796497 & ($20.30 \pm 0.01$, $18.55 \pm 0.00$, $17.94 \pm 0.00$, $17.61 \pm 0.00$, $17.48 \pm 0.01$) & $0.39 \pm 0.02$ \\
DESJ0604-3347 (1) & 91.062700 & -33.797510 & \ldots & \ldots \\
\hline
DESJ0610-5559A (A) & 92.681870 & -55.995240 & ($21.97 \pm 0.04$, $20.06 \pm 0.01$, $19.30 \pm 0.01$, $18.89 \pm 0.01$, $18.83 \pm 0.03$) & $0.51 \pm 0.02$ \\
DESJ0610-5559A (1) & 92.682600 & -55.994190 & ($22.50 \pm 0.05$, $21.43 \pm 0.02$, $20.62 \pm 0.02$, $20.20 \pm 0.02$, $20.38 \pm 0.08$) & $0.82 \pm 0.04$ \\
\hline
DESJ0610-5559B (A) & 92.681870 & -55.995240 & ($21.97 \pm 0.04$, $20.06 \pm 0.01$, $19.30 \pm 0.01$, $18.89 \pm 0.01$, $18.83 \pm 0.03$) & $0.51 \pm 0.02$ \\
DESJ0610-5559B (1) & 92.683290 & -55.992880 & ($21.95 \pm 0.03$, $21.37 \pm 0.02$, $21.11 \pm 0.03$, $20.97 \pm 0.05$, $21.20 \pm 0.19$) & $0.22 \pm 0.09$ \\
DESJ0610-5559B (2) & 92.680760 & -55.992680 & \ldots & \ldots \\
\hline
DESJ0611-5514A (A) & 92.987354 & -55.233840 & ($20.65 \pm 0.02$, $19.15 \pm 0.01$, $18.30 \pm 0.00$, $17.86 \pm 0.00$, $17.73 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.57 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0611-5514A (B) & 92.989168 & -55.232553 & ($21.13 \pm 0.02$, $19.72 \pm 0.01$, $18.88 \pm 0.01$, $18.44 \pm 0.01$, $18.31 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.58 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0611-5514A (1) & 92.987942 & -55.231195 & ($22.14 \pm 0.10$, $20.72 \pm 0.03$, $19.90 \pm 0.03$, $19.47 \pm 0.03$, $19.57 \pm 0.11$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.53 \pm 0.13$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0611-5514A (2) & 92.992356 & -55.234748 & ($22.08 \pm 0.10$, $21.04 \pm 0.04$, $20.42 \pm 0.05$, $20.29 \pm 0.07$, $20.37 \pm 0.22$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.63 \pm 0.41$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0611-5514A (3) & 92.987060 & -55.235893 & ($22.86 \pm 0.06$, $21.72 \pm 0.02$, $20.87 \pm 0.02$, $20.46 \pm 0.02$, $20.29 \pm 0.06$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.35 \pm 4.89$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ0611-5514B (A) & 92.987354 & -55.233840 & ($20.65 \pm 0.02$, $19.15 \pm 0.01$, $18.30 \pm 0.00$, $17.86 \pm 0.00$, $17.73 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.57 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0611-5514B (B) & 92.989168 & -55.232553 & ($21.13 \pm 0.02$, $19.72 \pm 0.01$, $18.88 \pm 0.01$, $18.44 \pm 0.01$, $18.31 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.58 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ0611-5514B (1) & 92.990120 & -55.234500 & ($21.81 \pm 0.12$, $20.61 \pm 0.05$, $19.88 \pm 0.05$, $19.69 \pm 0.08$, $19.78 \pm 0.23$)\textsuperscript{\textdagger} & $0.28 \pm 0.02$\textsuperscript{\textdagger} \\
DESJ0611-5514B (2) & 92.991190 & -55.232570 & ($22.76 \pm 0.12$, $21.95 \pm 0.07$, $21.40 \pm 0.09$, $21.06 \pm 0.13$, $21.01 \pm 0.30$)\textsuperscript{\textdagger} & $0.74 \pm 0.30$\textsuperscript{\textdagger} \\
DESJ0611-5514B (3) & 92.983520 & -55.232670 & ($22.92 \pm 0.11$, $22.56 \pm 0.10$, $22.19 \pm 0.14$, $22.05 \pm 0.25$, $21.44 \pm 0.35$)\textsuperscript{\textdagger} & $0.78 \pm 0.56$\textsuperscript{\textdagger} \\
\hline
DESJ0612-3920 (A) & 93.114428 & -39.343435 & ($21.20 \pm 0.03$, $19.71 \pm 0.01$, $19.05 \pm 0.01$, $18.67 \pm 0.01$, $18.63 \pm 0.04$)\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} & $0.51 \pm 0.01$\textsuperscript{\textdagger\fnsymbol{asteriskfootnote}} \\
DESJ0612-3920 (1) & 93.113140 & -39.343410 & \ldots & \ldots \\
\hline
DESJ2011-5725 (A) & 302.862410 & -57.419710 & ($18.92 \pm 0.01$, $17.48 \pm 0.00$, $17.00 \pm 0.00$, $16.68 \pm 0.00$, $16.53 \pm 0.01$)\textsuperscript{\textdagger} & $0.26 \pm 0.00$\textsuperscript{\textdagger} \\
DESJ2011-5725 (1) & 302.866640 & -57.422730 & ($22.17 \pm 0.06$, $21.43 \pm 0.05$, $21.28 \pm 0.08$, $20.90 \pm 0.09$, $21.67 \pm 0.75$)\textsuperscript{\textdagger} & $0.36 \pm 0.04$\textsuperscript{\textdagger} \\
\hline
\hline
DESJ2019-5642 (A) & 304.758838 & -56.711057 & ($99.00 \pm 99.00$, $16.78 \pm 0.00$, $16.31 \pm 0.00$, $15.96 \pm 0.00$, $15.82 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.11 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2019-5642 (1) & 304.754480 & -56.706860 & \ldots & \ldots \\
\hline
DESJ2022-6032 (A) & 305.691881 & -60.544299 & ($21.25 \pm 0.03$, $19.42 \pm 0.01$, $18.83 \pm 0.01$, $18.49 \pm 0.01$, $18.38 \pm 0.03$) & $0.36 \pm 0.02$ \\
DESJ2022-6032 (1) & 305.691385 & -60.546360 & ($21.39 \pm 0.02$, $20.69 \pm 0.02$, $20.48 \pm 0.02$, $20.45 \pm 0.04$, $20.34 \pm 0.14$) & $0.27 \pm 0.04$ \\
DESJ2022-6032 (2) & 305.695701 & -60.545406 & ($22.34 \pm 0.04$, $21.46 \pm 0.03$, $21.17 \pm 0.03$, $21.09 \pm 0.05$, $21.29 \pm 0.26$) & $0.47 \pm 0.12$ \\
\hline
DESJ2023-5535 (A) & 305.836987 & -55.597241 & ($18.49 \pm 0.01$, $17.08 \pm 0.00$, $16.59 \pm 0.00$, $16.28 \pm 0.00$, $16.18 \pm 0.01$) & $0.23 \pm 0.00$ \\
DESJ2023-5535 (1) & 305.840620 & -55.597490 & \ldots & \ldots \\
\hline
DESJ2028-4316 (A) & 307.170119 & -43.282161 & ($19.75 \pm 0.01$, $18.13 \pm 0.00$, $17.57 \pm 0.00$, $17.24 \pm 0.00$, $17.11 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.34 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2028-4316 (1) & 307.171026 & -43.283205 & ($22.29 \pm 0.04$, $20.55 \pm 0.01$, $19.73 \pm 0.01$, $19.29 \pm 0.01$, $19.12 \pm 0.03$) & $0.58 \pm 0.03$ \\
\hline
DESJ2031-4037 (A) & 307.971895 & -40.625215 & ($19.53 \pm 0.01$, $17.94 \pm 0.00$, $17.41 \pm 0.00$, $17.13 \pm 0.01$, $17.08 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.34 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2031-4037 (1) & 307.963336 & -40.623872 & ($23.08 \pm 0.21$, $21.52 \pm 0.07$, $21.03 \pm 0.08$, $20.87 \pm 0.12$, $22.34 \pm 1.55$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.57 \pm 0.18$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
\hline
DESJ2046-6146 (A) & 311.601910 & -61.782441 & ($19.41 \pm 0.01$, $17.78 \pm 0.00$, $17.21 \pm 0.00$, $16.88 \pm 0.00$, $16.73 \pm 0.02$) & $0.34 \pm 0.01$ \\
DESJ2046-6146 (1) & 311.605480 & -61.781700 & \ldots & \ldots \\
\hline
DESJ2106-4411 (A) & 316.529900 & -44.198250 & ($20.25 \pm 0.01$, $18.98 \pm 0.00$, $18.46 \pm 0.00$, $18.14 \pm 0.01$, $18.07 \pm 0.02$) & $0.36 \pm 0.02$ \\
DESJ2106-4411 (B) & 316.528440 & -44.197380 & ($20.99 \pm 0.01$, $19.60 \pm 0.01$, $18.98 \pm 0.00$, $18.61 \pm 0.01$, $18.51 \pm 0.02$) & $0.49 \pm 0.07$ \\
DESJ2106-4411 (C) & 316.528970 & -44.199260 & ($21.79 \pm 0.02$, $20.31 \pm 0.01$, $19.74 \pm 0.01$, $19.42 \pm 0.01$, $19.31 \pm 0.04$) & $0.41 \pm 0.08$ \\
DESJ2106-4411 (D) & 316.528560 & -44.198560 & ($21.41 \pm 0.01$, $19.95 \pm 0.00$, $19.38 \pm 0.00$, $19.05 \pm 0.01$, $18.94 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.35 \pm 0.07$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2106-4411 (1) & 316.531020 & -44.198880 & \ldots & \ldots \\
DESJ2106-4411 (2) & 316.527800 & -44.198900 & \ldots & \ldots \\
\hline
DESJ2112-4801 (A) & 318.088208 & -48.029790 & ($22.32 \pm 0.04$, $20.55 \pm 0.01$, $19.57 \pm 0.01$, $19.14 \pm 0.01$, $19.00 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.61 \pm 0.03$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2112-4801 (1) & 318.085648 & -48.030166 & ($21.26 \pm 0.04$, $20.64 \pm 0.03$, $20.38 \pm 0.05$, $20.14 \pm 0.07$, $19.71 \pm 0.19$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.19 \pm 0.15$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ2122-0059 (A) & 320.716650 & -0.997040 & ($20.15 \pm 0.01$, $19.06 \pm 0.01$, $18.52 \pm 0.01$, $18.21 \pm 0.01$, $18.11 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.35 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2122-0059 (1) & 320.717240 & -0.997630 & \ldots & \ldots \\
\hline
DESJ2124-6125 (A) & 321.112850 & -61.419530 & ($22.02 \pm 0.05$, $20.26 \pm 0.01$, $19.63 \pm 0.01$, $19.22 \pm 0.02$, $18.91 \pm 0.04$)\textsuperscript{\textdagger} & $0.47 \pm 0.03$\textsuperscript{\textdagger} \\
DESJ2124-6125 (1) & 321.114740 & -61.419040 & ($20.50 \pm 0.03$, $19.99 \pm 0.02$, $19.74 \pm 0.03$, $19.02 \pm 0.03$, $18.14 \pm 0.04$)\textsuperscript{\textdagger} & $0.50 \pm 0.02$\textsuperscript{\textdagger} \\
\hline
DESJ2131-4019 (A) & 322.770501 & -40.322545 & ($20.01 \pm 0.01$, $18.29 \pm 0.00$, $17.67 \pm 0.00$, $17.29 \pm 0.00$, $17.18 \pm 0.01$) & $0.35 \pm 0.02$ \\
DESJ2131-4019 (1) & 322.773428 & -40.318226 & ($21.31 \pm 0.04$, $20.54 \pm 0.03$, $20.09 \pm 0.03$, $19.78 \pm 0.05$, $19.49 \pm 0.13$) & $0.86 \pm 0.31$ \\
\hline
DESJ2134-4238 (A) & 323.502925 & -42.648129 & ($17.02 \pm 0.00$, $15.78 \pm 0.00$, $15.38 \pm 0.00$, $15.03 \pm 0.00$, $14.89 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.20 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2134-4238 (1) & 323.491570 & -42.645100 & \ldots & \ldots \\
\hline
DESJ2138-6007 (A) & 324.500308 & -60.131790 & ($18.94 \pm 0.00$, $17.36 \pm 0.00$, $16.83 \pm 0.00$, $16.51 \pm 0.00$, $16.35 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.30 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2138-6007 (B) & 324.503617 & -60.131615 & ($19.59 \pm 0.00$, $17.95 \pm 0.00$, $17.41 \pm 0.00$, $17.07 \pm 0.00$, $16.94 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.30 \pm 0.05$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2138-6007 (1) & 324.515840 & -60.130450 & \ldots & \ldots \\
DESJ2138-6007 (2) & 324.514900 & -60.135570 & \ldots & \ldots \\
DESJ2138-6007 (3) & 324.497250 & -60.129370 & \ldots & \ldots \\
DESJ2138-6007 (4) & 324.495360 & -60.137310 & \ldots & \ldots \\
\hline
DESJ2139-4251 (A) & 324.780198 & -42.861517 & ($21.04 \pm 0.02$, $20.05 \pm 0.01$, $19.51 \pm 0.01$, $19.18 \pm 0.02$, $19.13 \pm 0.05$)\textsuperscript{\textdagger} & $0.57 \pm 0.02$\textsuperscript{\textdagger} \\
DESJ2139-4251 (1) & 324.780331 & -42.860736 & ($21.91 \pm 0.02$, $21.47 \pm 0.02$, $21.18 \pm 0.03$, $20.95 \pm 0.04$, $21.09 \pm 0.14$)\textsuperscript{\textdagger} & $0.79 \pm 0.04$\textsuperscript{\textdagger} \\
\hline
DESJ2144-4323 (A) & 326.010515 & -43.396510 & ($19.10 \pm 0.00$, $17.60 \pm 0.00$, $17.12 \pm 0.00$, $16.80 \pm 0.00$, $16.64 \pm 0.00$) & $0.27 \pm 0.01$ \\
DESJ2144-4323 (1) & 326.012910 & -43.397770 & \ldots & \ldots \\
\hline
DESJ2145-5644 (A) & 326.466620 & -56.748122 & ($19.64 \pm 0.01$, $18.24 \pm 0.00$, $17.64 \pm 0.00$, $17.27 \pm 0.01$, $17.11 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.30 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2145-5644 (1) & 326.477890 & -56.753000 & \ldots & \ldots \\
DESJ2145-5644 (2) & 326.467700 & -56.756310 & \ldots & \ldots \\
\hline
DESJ2152-5555 (A) & 328.035960 & -55.927460 & ($20.76 \pm 0.02$, $19.87 \pm 0.01$, $19.53 \pm 0.02$, $19.13 \pm 0.02$, $18.56 \pm 0.05$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.37 \pm 0.14$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2152-5555 (1) & 328.035020 & -55.928180 & \ldots & \ldots \\
\hline
DESJ2154-4604 (A) & 328.686468 & -46.074771 & ($21.70 \pm 0.05$, $20.01 \pm 0.01$, $19.23 \pm 0.01$, $18.81 \pm 0.01$, $18.72 \pm 0.04$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.61 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2154-4604 (1) & 328.687346 & -46.073872 & ($22.62 \pm 0.10$, $21.12 \pm 0.03$, $20.80 \pm 0.04$, $20.67 \pm 0.06$, $20.62 \pm 0.22$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.41 \pm 0.08$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ2157-5700 (A) & 329.476090 & -57.009240 & ($21.70 \pm 0.02$, $19.96 \pm 0.01$, $19.28 \pm 0.01$, $18.88 \pm 0.01$, $18.75 \pm 0.03$)\textsuperscript{\textdagger} & $0.41 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ2157-5700 (1) & 329.477010 & -57.008060 & \ldots & \ldots \\
\hline
DESJ2159-6245 (A) & 329.994485 & -62.753882 & ($19.93 \pm 0.01$, $18.28 \pm 0.00$, $17.70 \pm 0.00$, $17.37 \pm 0.01$, $17.22 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.37 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2159-6245 (1) & 329.997400 & -62.752930 & \ldots & \ldots \\
\hline
DESJ2200-4128 (A) & 330.185470 & -41.472300 & ($21.31 \pm 0.02$, $20.47 \pm 0.01$, $19.79 \pm 0.01$, $19.35 \pm 0.02$, $19.24 \pm 0.05$) & $0.63 \pm 0.04$ \\
DESJ2200-4128 (1) & 330.185070 & -41.471840 & \ldots & \ldots \\
\hline
DESJ2201-5956 (A) & 330.472324 & -59.945410 & ($16.69 \pm 0.00$, $15.72 \pm 0.00$, $15.28 \pm 0.00$, $14.95 \pm 0.00$, $14.80 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.10 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2201-5956 (1) & 330.481090 & -59.948430 & \ldots & \ldots \\
\hline
DESJ2219-4348 (A) & 334.801660 & -43.809750 & ($21.41 \pm 0.03$, $20.13 \pm 0.02$, $19.10 \pm 0.01$, $18.67 \pm 0.01$, $18.49 \pm 0.03$)\textsuperscript{\textdagger} & $0.71 \pm 0.02$\textsuperscript{\textdagger} \\
DESJ2219-4348 (1) & 334.801150 & -43.810470 & \ldots & \ldots \\
DESJ2219-4348 (2) & 334.802630 & -43.810380 & \ldots & \ldots \\
\hline
DESJ2223-6329 (A) & 335.921335 & -63.492151 & ($22.01 \pm 0.04$, $20.39 \pm 0.01$, $19.39 \pm 0.01$, $18.96 \pm 0.01$, $18.82 \pm 0.03$) & $0.67 \pm 0.02$ \\
DESJ2223-6329 (1) & 335.918953 & -63.491625 & ($22.02 \pm 0.05$, $20.97 \pm 0.03$, $20.55 \pm 0.03$, $20.42 \pm 0.05$, $20.06 \pm 0.13$) & $0.53 \pm 0.13$ \\
DESJ2223-6329 (2) & 335.920408 & -63.493589 & ($23.16 \pm 0.09$, $22.04 \pm 0.05$, $21.81 \pm 0.06$, $21.66 \pm 0.11$, $22.53 \pm 0.85$) & $0.55 \pm 0.06$ \\
\hline
DESJ2232-5807 (A) & 338.237280 & -58.128650 & ($21.36 \pm 0.03$, $19.65 \pm 0.01$, $18.72 \pm 0.01$, $18.32 \pm 0.01$, $18.17 \pm 0.02$)\textsuperscript{\textdagger} & $0.59 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ2232-5807 (1) & 338.239240 & -58.130650 & ($21.20 \pm 0.02$, $20.78 \pm 0.02$, $20.51 \pm 0.03$, $20.41 \pm 0.04$, $20.27 \pm 0.11$)\textsuperscript{\textdagger} & $0.10 \pm 0.00$\textsuperscript{\textdagger} \\
\hline
DESJ2232-5959 (A) & 338.140910 & -59.998120 & ($20.98 \pm 0.02$, $19.36 \pm 0.01$, $18.48 \pm 0.00$, $18.05 \pm 0.01$, $17.93 \pm 0.02$) & $0.58 \pm 0.01$ \\
DESJ2232-5959 (1) & 338.144720 & -59.999420 & ($22.35 \pm 0.02$, $22.00 \pm 0.02$, $21.38 \pm 0.02$, $21.08 \pm 0.03$, $21.16 \pm 0.11$) & $0.98 \pm 0.09$ \\
DESJ2232-5959 (2) & 338.140850 & -60.000570 & \ldots & \ldots \\
\hline
DESJ2233-0104 (A) & 338.320060 & -1.069414 & ($23.88 \pm 0.28$, $21.81 \pm 0.05$, $20.64 \pm 0.03$, $19.93 \pm 0.03$, $19.74 \pm 0.08$) & $0.89 \pm 0.04$ \\
DESJ2233-0104 (1) & 338.320128 & -1.067883 & ($23.02 \pm 0.13$, $22.17 \pm 0.07$, $21.42 \pm 0.06$, $21.22 \pm 0.10$, $21.62 \pm 0.48$) & $0.97 \pm 0.09$ \\
DESJ2233-0104 (2) & 338.319234 & -1.068397 & ($24.86 \pm 0.50$, $24.13 \pm 0.31$, $22.97 \pm 0.19$, $22.47 \pm 0.22$, $22.00 \pm 0.47$) & $1.05 \pm 0.21$ \\
\hline
DESJ2240-5245 (A) & 340.249290 & -52.754180 & ($18.27 \pm 0.00$, $16.98 \pm 0.00$, $16.54 \pm 0.00$, $16.22 \pm 0.00$, $16.10 \pm 0.01$) & $0.22 \pm 0.01$ \\
DESJ2240-5245 (1) & 340.252120 & -52.754230 & \ldots & \ldots \\
\hline
DESJ2254-4620 (A) & 343.585510 & -46.346820 & ($18.41 \pm 0.00$, $16.96 \pm 0.00$, $16.50 \pm 0.00$, $16.19 \pm 0.00$, $16.03 \pm 0.01$)\textsuperscript{\textdagger} & $0.27 \pm 0.00$\textsuperscript{\textdagger} \\
DESJ2254-4620 (1) & 343.584430 & -46.336430 & ($20.81 \pm 0.04$, $19.86 \pm 0.02$, $19.50 \pm 0.03$, $19.28 \pm 0.05$, $19.02 \pm 0.09$)\textsuperscript{\textdagger} & $0.28 \pm 0.02$\textsuperscript{\textdagger} \\
DESJ2254-4620 (2) & 343.598880 & -46.346170 & ($21.63 \pm 0.04$, $20.72 \pm 0.02$, $20.06 \pm 0.02$, $19.74 \pm 0.05$, $19.66 \pm 0.09$)\textsuperscript{\textdagger} & $0.69 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ2254-4620 (3) & 343.596580 & -46.349810 & \ldots & \ldots \\
\hline
DESJ2300-5820 (A) & 345.239077 & -58.349701 & ($22.34 \pm 0.05$, $20.39 \pm 0.01$, $19.41 \pm 0.01$, $18.98 \pm 0.01$, $18.91 \pm 0.03$) & $0.62 \pm 0.02$ \\
DESJ2300-5820 (1) & 345.238774 & -58.347404 & ($22.56 \pm 0.04$, $22.06 \pm 0.04$, $21.78 \pm 0.06$, $21.67 \pm 0.10$, $21.19 \pm 0.20$) & $0.63 \pm 0.48$ \\
DESJ2300-5820 (2) & 345.237410 & -58.347707 & ($22.90 \pm 0.04$, $22.43 \pm 0.04$, $22.28 \pm 0.06$, $22.17 \pm 0.10$, $22.67 \pm 0.51$) & $0.34 \pm 0.26$ \\
\hline
DESJ2308-0155 (A) & 347.003815 & -1.928142 & ($19.74 \pm 0.01$, $18.13 \pm 0.00$, $17.57 \pm 0.00$, $17.22 \pm 0.00$, $17.05 \pm 0.01$) & $0.28 \pm 0.01$ \\
DESJ2308-0155 (1) & 347.006057 & -1.928119 & ($19.96 \pm 0.03$, $18.70 \pm 0.01$, $18.22 \pm 0.02$, $18.07 \pm 0.02$, $17.82 \pm 0.06$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.20 \pm 0.06$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ2308-0211 (A) & 347.092550 & -2.192137 & ($18.92 \pm 0.01$, $17.28 \pm 0.00$, $16.74 \pm 0.00$, $16.40 \pm 0.00$, $16.21 \pm 0.01$)\textsuperscript{\textdagger} & $0.26 \pm 0.00$\textsuperscript{\textdagger} \\
DESJ2308-0211 (1) & 347.084109 & -2.186774 & ($22.04 \pm 0.12$, $20.80 \pm 0.06$, $20.09 \pm 0.05$, $19.78 \pm 0.07$, $19.78 \pm 0.21$)\textsuperscript{\textdagger} & $0.69 \pm 0.05$\textsuperscript{\textdagger} \\
\hline
DESJ2311-6307 (A) & 347.990373 & -63.117555 & ($21.79 \pm 0.03$, $20.70 \pm 0.01$, $19.86 \pm 0.01$, $19.34 \pm 0.01$, $19.06 \pm 0.04$) & $0.75 \pm 0.04$ \\
DESJ2311-6307 (1) & 347.991865 & -63.117135 & ($21.76 \pm 0.02$, $21.08 \pm 0.02$, $20.74 \pm 0.02$, $20.51 \pm 0.03$, $20.52 \pm 0.12$) & $0.49 \pm 0.16$ \\
\hline
DESJ2322-6409 (A) & 350.682710 & -64.165650 & ($19.19 \pm 0.00$, $17.82 \pm 0.00$, $17.35 \pm 0.00$, $17.02 \pm 0.00$, $16.88 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.25 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2322-6409 (B) & 350.681260 & -64.165230 & ($18.69 \pm 0.00$, $17.24 \pm 0.00$, $16.77 \pm 0.00$, $16.45 \pm 0.00$, $16.31 \pm 0.00$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.25 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2322-6409 (1) & 350.676660 & -64.165080 & ($18.77 \pm 0.01$, $17.55 \pm 0.00$, $17.13 \pm 0.00$, $16.82 \pm 0.00$, $16.58 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.11 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2322-6409 (2) & 350.677500 & -64.166460 & \ldots & \ldots \\
\hline
DESJ2324-4944 (A) & 351.136170 & -49.749430 & ($22.07 \pm 0.04$, $20.19 \pm 0.01$, $19.29 \pm 0.01$, $18.89 \pm 0.01$, $18.78 \pm 0.03$) & $0.58 \pm 0.02$ \\
DESJ2324-4944 (1) & 351.137390 & -49.750640 & ($22.17 \pm 0.09$, $21.22 \pm 0.05$, $20.56 \pm 0.05$, $20.42 \pm 0.07$, $19.95 \pm 0.15$) & $0.82 \pm 0.17$ \\
DESJ2324-4944 (2) & 351.138280 & -49.749640 & ($22.11 \pm 0.08$, $21.08 \pm 0.04$, $20.50 \pm 0.04$, $20.42 \pm 0.07$, $19.88 \pm 0.12$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.67 \pm 0.67$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ2325-4111 (A) & 351.300070 & -41.199060 & ($19.49 \pm 0.02$, $17.78 \pm 0.00$, $17.24 \pm 0.01$, $16.94 \pm 0.01$, $16.77 \pm 0.02$)\textsuperscript{\textdagger} & $0.35 \pm 0.00$\textsuperscript{\textdagger} \\
DESJ2325-4111 (1) & 351.296950 & -41.187470 & ($21.25 \pm 0.02$, $21.19 \pm 0.03$, $21.22 \pm 0.05$, $20.93 \pm 0.05$, $20.73 \pm 0.12$)\textsuperscript{\textdagger} & $0.55 \pm 0.10$\textsuperscript{\textdagger} \\
DESJ2325-4111 (2) & 351.292710 & -41.188740 & ($20.83 \pm 0.04$, $20.63 \pm 0.05$, $20.52 \pm 0.08$, $20.19 \pm 0.07$, $20.27 \pm 0.22$)\textsuperscript{\textdagger} & $1.58 \pm 0.00$\textsuperscript{\textdagger} \\
\hline
DESJ2331-5051 (A) & 352.963120 & -50.864987 & ($21.46 \pm 0.02$, $19.65 \pm 0.01$, $18.73 \pm 0.00$, $18.31 \pm 0.01$, $18.18 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.59 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2331-5051 (1) & 352.959700 & -50.860790 & \ldots & \ldots \\
DESJ2331-5051 (2) & 352.964380 & -50.860420 & \ldots & \ldots \\
\hline
DESJ2332-0152 (A) & 353.004387 & -1.868152 & ($19.89 \pm 0.00$, $19.61 \pm 0.00$, $19.45 \pm 0.00$, $19.38 \pm 0.01$, $19.33 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.08 \pm 0.12$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2332-0152 (1) & 353.004510 & -1.868758 & ($20.03 \pm 0.00$, $20.15 \pm 0.01$, $20.07 \pm 0.01$, $20.23 \pm 0.02$, $20.21 \pm 0.06$) & $0.05 \pm 0.42$ \\
DESJ2332-0152 (2) & 353.005267 & -1.867614 & ($19.83 \pm 0.00$, $20.13 \pm 0.01$, $20.08 \pm 0.01$, $20.38 \pm 0.02$, $20.31 \pm 0.07$) & $0.05 \pm 0.23$ \\
DESJ2332-0152 (3) & 353.004633 & -1.866993 & ($20.97 \pm 0.01$, $21.02 \pm 0.01$, $20.86 \pm 0.01$, $21.06 \pm 0.03$, $20.86 \pm 0.09$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.31 \pm 0.77$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline
DESJ2335-4209 (A) & 353.841368 & -42.152276 & ($20.44 \pm 0.01$, $18.84 \pm 0.00$, $18.15 \pm 0.00$, $17.77 \pm 0.01$, $17.63 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.49 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2335-4209 (1) & 353.841520 & -42.153450 & \ldots & \ldots \\
\hline
DESJ2335-5152 (A) & 353.966419 & -51.871635 & ($20.83 \pm 0.02$, $19.45 \pm 0.01$, $18.66 \pm 0.01$, $18.28 \pm 0.01$, $18.14 \pm 0.02$) & $0.57 \pm 0.02$ \\
DESJ2335-5152 (1) & 353.966070 & -51.872742 & ($21.76 \pm 0.02$, $21.16 \pm 0.01$, $20.74 \pm 0.02$, $20.39 \pm 0.02$, $20.13 \pm 0.06$) & $0.64 \pm 0.22$ \\
DESJ2335-5152 (2) & 353.967170 & -51.870870 & \ldots & \ldots \\
\hline
DESJ2336-5352 (A) & 354.029770 & -53.876660 & ($20.50 \pm 0.01$, $18.83 \pm 0.00$, $18.07 \pm 0.00$, $17.67 \pm 0.00$, $17.51 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.52 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2336-5352 (1) & 354.032790 & -53.878140 & ($21.64 \pm 0.06$, $20.78 \pm 0.03$, $19.99 \pm 0.03$, $19.75 \pm 0.05$, $19.37 \pm 0.11$) & $0.81 \pm 0.05$ \\
DESJ2336-5352 (2) & 354.027830 & -53.876300 & ($21.77 \pm 0.03$, $20.89 \pm 0.01$, $20.26 \pm 0.01$, $19.77 \pm 0.02$, $19.57 \pm 0.05$) & $0.94 \pm 0.08$ \\
\hline
DESJ2341-5716 (A) & 355.272785 & -57.267740 & ($19.64 \pm 0.01$, $18.19 \pm 0.00$, $17.60 \pm 0.00$, $17.20 \pm 0.00$, $17.07 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.36 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2341-5716 (1) & 355.276978 & -57.267172 & ($21.22 \pm 0.09$, $19.50 \pm 0.03$, $18.96 \pm 0.03$, $18.61 \pm 0.04$, $18.46 \pm 0.10$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $-0.00 \pm 0.10$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2341-5716 (2) & 355.269310 & -57.266230 & \ldots & \ldots \\
\hline
DESJ2342-4652 (A) & 355.650095 & -46.874445 & ($18.55 \pm 0.00$, $17.18 \pm 0.00$, $16.73 \pm 0.00$, $16.41 \pm 0.00$, $16.25 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.27 \pm 0.01$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2342-4652 (1) & 355.651120 & -46.876340 & \ldots & \ldots \\
\hline
DESJ2343-6039 (A) & 355.865374 & -60.650262 & ($22.19 \pm 0.06$, $20.35 \pm 0.02$, $19.34 \pm 0.01$, $18.93 \pm 0.01$, $18.74 \pm 0.04$)\textsuperscript{\textdagger} & $0.64 \pm 0.01$\textsuperscript{\textdagger} \\
DESJ2343-6039 (1) & 355.871630 & -60.650622 & ($23.42 \pm 0.14$, $22.60 \pm 0.10$, $22.18 \pm 0.12$, $22.04 \pm 0.19$, $21.41 \pm 0.31$)\textsuperscript{\textdagger} & $1.02 \pm 0.09$\textsuperscript{\textdagger} \\
\hline
DESJ2347-6246 (A) & 356.789415 & -62.776592 & ($18.70 \pm 0.00$, $17.43 \pm 0.00$, $16.99 \pm 0.00$, $16.69 \pm 0.00$, $16.57 \pm 0.01$) & $0.23 \pm 0.01$ \\
DESJ2347-6246 (1) & 356.786300 & -62.777610 & \ldots & \ldots \\
\hline
DESJ2347-6245 (A) & 356.802592 & -62.765895 & ($18.38 \pm 0.00$, $17.00 \pm 0.00$, $16.54 \pm 0.00$, $16.24 \pm 0.00$, $16.14 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.24 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2347-6245 (1) & 356.800980 & -62.768670 & \ldots & \ldots \\
\hline
DESJ2349-5113 (A) & 357.375315 & -51.227540 & ($19.53 \pm 0.01$, $18.03 \pm 0.00$, $17.48 \pm 0.00$, $17.12 \pm 0.00$, $16.99 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.39 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2349-5113 (1) & 357.373786 & -51.227103 & ($21.99 \pm 0.01$, $21.38 \pm 0.01$, $21.04 \pm 0.01$, $20.65 \pm 0.01$, $20.48 \pm 0.03$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.46 \pm 0.28$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2349-5113 (2) & 357.374390 & -51.228910 & \ldots & \ldots \\
DESJ2349-5113 (3) & 357.377180 & -51.227180 & \ldots & \ldots \\
\hline
DESJ2351-5452 (A) & 357.908633 & -54.881696 & ($19.51 \pm 0.01$, $17.83 \pm 0.00$, $17.25 \pm 0.00$, $16.93 \pm 0.00$, $16.80 \pm 0.01$) & $0.38 \pm 0.01$ \\
DESJ2351-5452 (1) & 357.907948 & -54.880073 & ($20.91 \pm 0.03$, $19.71 \pm 0.01$, $19.18 \pm 0.01$, $18.95 \pm 0.02$, $18.95 \pm 0.06$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.58 \pm 0.16$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2351-5452 (2) & 357.911524 & -54.882907 & ($21.59 \pm 0.02$, $20.65 \pm 0.01$, $20.10 \pm 0.01$, $19.84 \pm 0.02$, $19.71 \pm 0.05$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.16 \pm 1.04$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2351-5452 (3) & 357.907370 & -54.884050 & \ldots & \ldots \\
\hline
DESJ2358-6125 (A) & 359.700322 & -61.433041 & ($19.70 \pm 0.01$, $18.06 \pm 0.00$, $17.49 \pm 0.00$, $17.14 \pm 0.00$, $16.96 \pm 0.02$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.39 \pm 0.02$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2358-6125 (1) & 359.698720 & -61.434140 & \ldots & \ldots \\
\hline
DESJ2359+0208 (A) & 359.889732 & 2.139907 & ($19.46 \pm 0.01$, $17.60 \pm 0.00$, $16.98 \pm 0.00$, $16.59 \pm 0.00$, $16.43 \pm 0.01$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.43 \pm 0.00$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2359+0208 (1) & 359.891845 & 2.140704 & ($21.99 \pm 0.08$, $20.01 \pm 0.02$, $19.36 \pm 0.01$, $18.87 \pm 0.02$, $18.78 \pm 0.06$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.26 \pm 0.13$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
DESJ2359+0208 (2) & 359.891906 & 2.138341 & ($23.02 \pm 0.09$, $21.47 \pm 0.03$, $20.71 \pm 0.02$, $19.98 \pm 0.02$, $20.01 \pm 0.09$)\textsuperscript{\fnsymbol{asteriskfootnote}} & $0.82 \pm 0.06$\textsuperscript{\fnsymbol{asteriskfootnote}} \\
\hline

